How Effective are Smart Contract Analysis Tools? Evaluating Smart Contract Static Analysis Tools Using Bug Injection

Security attacks targeting smart contracts have been on the rise, which have led to financial loss and erosion of trust. Therefore, it is important to enable developers to discover security vulnerabilities in smart contracts before deployment. A number of static analysis tools have been developed for finding security bugs in smart contracts. However, despite the numerous bug-finding tools, there is no systematic approach to evaluate the proposed tools and gauge their effectiveness. This paper proposes SolidiFI, an automated and systematic approach for evaluating smart contract static analysis tools. SolidiFI is based on injecting bugs (i.e., code defects) into all potential locations in a smart contract to introduce targeted security vulnerabilities. SolidiFI then checks the generated buggy contract using the static analysis tools, and identifies the bugs that the tools are unable to detect (false-negatives) along with identifying the bugs reported as false-positives. SolidiFI is used to evaluate six widely-used static analysis tools, namely, Oyente, Securify, Mythril, SmartCheck, Manticore and Slither, using a set of 50 contracts injected by 9369 distinct bugs. It finds several instances of bugs that are not detected by the evaluated tools despite their claims of being able to detect such bugs, and all the tools report many false positives

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.


==> SolidiFI-arXiv (2)/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> SolidiFI-arXiv (2)/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.


==> SolidiFI-arXiv (2)/abstract.tex <==
\pdfoutput=1

Security attacks targeting smart contracts have been on the rise, which have led to financial loss and erosion of trust.
%, creating huge consternation among smart contracts’ end-users. Code
Therefore, it is important to enable developers to discover security vulnerabilities in smart contracts before deployment. %, where several approaches have been proposed and a 
A number of static analysis tools have been developed for finding security bugs in smart contracts. However, despite the numerous bug-finding tools, there is no systematic approach to evaluate the proposed tools and gauge their effectiveness. 
This paper proposes \sysname, an automated and systematic approach for evaluating smart contracts' static analysis tools. \sysname is based on injecting bugs (i.e., code defects) into all potential locations in a smart contract to introduce targeted security vulnerabilities. \sysname then checks the generated buggy contract using the static analysis tools, and identifies the bugs that the tools are unable to detect (false-negatives) along with identifying the bugs reported as false-positives. \sysname is used to evaluate six widely-used static analysis tools, namely, Oyente, Securify, Mythril, SmartCheck, Manticore and Slither,  using a set of 50 contracts injected by 9369 distinct bugs. It finds several instances of bugs that are not detected by the evaluated tools despite their claims of being able to detect such bugs, and all the tools report many false positives. 

%Results show the applicability of the proposed approach in finding several security bugs belonging to different bug types were not detected by the evaluated tools.

==> SolidiFI-arXiv (2)/algorithm.tex <==
\pdfoutput=1

\section{\sysname Algorithm} 
\label{sec:algorithm}

%This section explains the  main algorithm of \textit{\sysname}. 
The process for injecting bugs takes as input the Abstract Syntax Tree (AST) of the smart contract, and has the following steps.
\begin{enumerate}
   % \item Compile a version of the target contract and generate the Abstract Syntax Tree (AST).
    \item Identify the potential locations for injecting bugs and generate an annotated AST marking all identified locations.
    \item Inject bugs into all marked locations to generate the buggy contract.
    \item Check the buggy contract using the evaluated tools and inspect the results for undetected bugs and false alarms.
\end{enumerate}
%Algorithm \ref{alg:solidifi} provides a high-level description of the algorithm.
We discuss the steps in detail below.

%\begin{figure}[h] 
%\centering
%\includegraphics[width=0.75\columnwidth]{figures/solidifi.eps}
%\caption{\sysname Components}
%\label{fig:solidifi}
%\end{figure}

%\begin{algorithm}[h]
%\algsetup{linenosize=\tiny}
%\caption{\sysname High-level Algorithm}
%\label{alg:solidifi}
%\small
%\begin{algorithmic}[1]
%\Procedure{main}{}
%\State $AST \gets Parser(contract.sol)$
%\For{Each bug type}
%\State $FIP \gets Find All Potential Locations(AST, bug)$
%\For{Each location in FIP}
 %\State{Decide injection approach}
% \If{approach  == inject snippet}
%    \State{Inject matching fault snippet}
%  \ElsIf{approach  == weaken security}
%  \State{Weaken existing security mechanism}
%  \ElsIf{approach  == transform code}
%    \State{Do required code transformation}
%  \EndIf
% \State{Record injection details in FaultLog}
% \EndFor
% \EndFor
% \For{Each tool being evaluated}
%  \State $Result \gets Check(buggyContract)$
%  \State $Undetected Faults \gets Inspect(result)$
% \EndFor
%\EndProcedure
%\end{algorithmic}
%\end{algorithm}
%\normalsize

%\textbf{Abstract syntax tree generation:}
%First, \sysname reads the source code of the target contract. Then the abstract syntax tree (AST) of the  target contract is generated.
%(line 2 in Algorithm \ref{alg:solidifi}).

\textbf{Bug locations identification:}
The AST is passed to \textit{Bug Locations Identifier}, that drives a bug injection profile (BIP) of all possible injection locations in the target contract for a given security bug. 
%(line 4 in Algorithm \ref{alg:solidifi}).
The BIP is derived using AST-based analysis for identifying potential injection locations in smart contract code by Algorithm \ref{alg:findlocs}. Algorithm \ref{alg:findlocs} takes as input the AST and the bug type to be injected, and outputs the BIP.

\begin{algorithm}[h]
%\algsetup{linenosize=\tiny}
\caption{Identifying Injection Locations Algorithm}
\label{alg:findlocs}
\small
\begin{algorithmic}[1]
\Procedure{FindAllPotentialLocations}{AST, bugType}
\For {Each form of code snippets in bugType}
    \If{snippetForm  == simple statement}
        \State $BIP \gets WalkAST(simpleStatement)$
    \ElsIf{snippetForm  == non-function block}
        \State $BIP \gets WalkAST(nonFunctionBlock)$
    \ElsIf {snippetForm  == functionDefinition}
        \State $BIP \gets WalkAST(functionDefinition)$
  \EndIf
 \EndFor
  \State $BIP \gets Find Related Security Mechanisms$
  \State $BIP \gets Find Code That Can Be Transformed$
 \State{return $BIP$}
 \EndProcedure
\end{algorithmic}
%\vspace{-4mm}
\end{algorithm}
\normalsize

To address the first challenge of identifying bug injection locations as mentioned in Section \ref{injectionchallenges}, we define rules that specify the relation between the bug to be injected and the target contract structure. In general, bugs take two forms: an individual statement, and a block of statements. A block of statements can be defined either as a stand-alone function, or a non-function block such as an 'if' statement. Therefore, we use a rule for each form of the bug that defines the specifications of the locations for injecting it. %For example, the specifications of the locations for injecting a bug formulated as a stand-alone function would be any location that is within the body of the contract, and not inside the body of another function or block of statements. 

To identify such locations, for each distinct form of the code snippets defining the bug type to be injected, we walk the AST based on the code snippet form and the related rule (lines 2-10 in Algorithm \ref{alg:findlocs}). $WalkAST(simpleStatement)$, for example, will visit (parse) the AST and find all the locations where a simple statement can be injected without invalidating the compilation state of the contract, and the same for the other forms of the code snippets of the bug type. After identifying the locations for injecting code snippets of bugs, we also look for existing security mechanisms to be weakened to introduce the related bug, and the code patterns to be transformed for introducing the bug (lines 11 and 12). %in Algorithm \ref{alg:findlocs}).

\textbf{Bug injection and code transformation:}
\sysname uses a systematic approach to inject bugs into the potential locations in the target contract. %(lines 6-13 in Algorithm \ref{alg:solidifi}).  
The \textit{Bug Injector} model seeds a bug for each location specified in the BIP. It uses text-based code transformation to modify the code where the information derived from the AST is used to modify the code to inject bugs.
Three different approaches are used to inject bugs as discussed in Section \ref{buginstrument}. In addition to injecting bugs in the target contract, \textit{Bug Injector} generates a \textit {BugLog} that specifies a unique identifier for each injected bug, and the corresponding location(s) in the target contract where it has been injected. % (line 14 in Algorithm \ref{alg:solidifi}).
%The \textit{FaultLog} is used for performing automated inspection of the results generated by the evaluated tools.

\textbf{Buggy code check and results inspection:}
The resulting buggy contract is passed to the \textit{Tool Evaluator} that checks the buggy code using the tools under evaluation. %(line 18 in Algorithm \ref{alg:solidifi}).
It then scans the results generated by the tools looking for the bugs that were injected but undetected, with the help of \textit{BugLog} generated by the \textit{Bug Injector}. %(line 19 in Algorithm \ref{alg:solidifi})
%and outputs the list of undetected bugs. 
\sysname only considers the injected bugs that are undetected. So if an evaluated tool reported bugs in locations other than where bugs have been injected, \sysname does not consider them in its output of false negatives. 
This is to avoid potential vulnerabilities in the original contract from being reported by \sysname, which would skew the results. Moreover, \sysname inspects results generated by the tools looking for other reported bugs and checks if they are true bugs or false alarms (more details in Section~\ref{sec:eva}).

\section{Implementation}
\label{sec:imp}
\sysname approach is fully-automated (except for the pre-prepared buggy snippets). This involves compiling the code, injecting and generating buggy contracts, running the evaluated tools on the buggy contracts, and inspecting reports of the evaluated tools for false-negatives, mis-identified cases, and false-positives (except for the manual validation of the filtered false-positives).
To make \sysname reusable, we did not hard-code the patterns that are replaced to introduce bugs, but rather made them configurable from an external file. We have made {\em \sysname code publicly available}\footnote{
		\url{https://github.com/DependableSystemsLab/SolidiFI} }. 


\sysname uses the Solidity compiler \textbf{solc} (supports compiler versions up to 0.5.12) to compile the source code of the smart contract to make sure it is free from compilation errors before bugs are injected. In addition, \sysname uses \textbf{solc} to generate the AST of the original code in JavaScript Object Notation (JSON) format. We have implemented the other components of \sysname in Python in about $1500$ lines of code. These components are responsible for identifying the potential locations for injection, injecting bugs using a suitable approach, generating the buggy contract, and inspecting the results of the evaluated tools and then reporting the undetected bugs and false alarms. Finally, we developed a Python client to interact with contracts deployed on Ethereum network - this client is used for assessing the exploitability of the injected bugs in the generated buggy contracts. 

%\sysname allows users to define the code patterns that are replaced, and the vulnerable patterns for each bug type.

==> SolidiFI-arXiv (2)/background.tex <==
\pdfoutput=1

\section{Background}
\label{sec:background}

%This section overviews Ethereum smart contracts, and the five security analysis tools considered in this work.

\subsection{Smart Contracts}
%Ethereum is a distributed-based computing platform running programs,
%called smart contracts. Smart contracts govern the behavior of accounts within the Ethereum state \cite{solidity1}, and are executed upon request of users. 
%Similar to traditional programs, in Ethereum, contracts are defined by a set of functions, each consisting of a sequence of transactions.
%
As mentioned earlier, smart contracts are written in a high-level language such as Solidity. They are compiled to Ethereum Virtual Machine (EVM) bytecode that is deployed and stored in the blockchain accounts. Smart contract transactions are executed by miners, which are a network of mutually untrusted nodes, and governed by the consensus protocol of the blockchain. Miners receive execution fees, called gas, for running the transactions which are paid by the users who submit the execution requests. We illustrate smart contracts through a running example shown in Figure~\ref{fig:example-contract} (adapted from prior work~\cite{atzei2017survey}). %, and is used as a running example in the paper. 

%\setlength{\floatsep}{1pt}
\begin{figure}[h]
\footnotesize
\centering
\begin{lstlisting}[language= Solidity, basicstyle=\ttfamily]
pragma solidity >=0.4.21 <0.6.0;
contract EGame{
    address payable private winner;
    uint startTime;
    
    constructor() public{ 
      winner = msg.sender;
      startTime = block.timestamp;}
    
    function play(bytes32 guess) public {
     if(keccak256(abi.encode(guess)) == keccak256(abi.encode('solution'))){
        if (startTime + (5 * 1 days) == block.timestamp){
           winner = msg.sender;}}}
           
    function getReward() payable public{
      winner.transfer(msg.value);}
 }    
\end{lstlisting}
\caption{Simple contract written in Solidity.}
\label{fig:example-contract}
%\vspace{-5mm}
\end{figure}

This contract implements a public game that enables users to play a game and submit their guesses or solutions for the game along with some amount of money. The money will be transferred to the account of the last winner if the guess is wrong; otherwise the user will be set as the current winner and will receive the money from users who play later. The \textit{constructor()} at line 6 runs only once when the contract is created, and it sets the initial winner to the owner of the contract defined by the user who submitted the create transaction of the contract (\textit{msg.sender}). It also initializes the \textit{startTime} variable to the current timestamp during the contract creation. The function \textit{play} at line 10 is called by the user who wants to submit his/her guess, and it compares the received guess with the true guess value. If the comparison is successful, it sets the \textit{winner} to the address of the user account who called this function, provided the guess was submitted within 5 days of creating the contract. Finally, the function \textit{getReward} sends the amount of \textit{ether} specified in the call to getReward (\textit{msg.value)}, to the last winner.


\subsection{Static Analysis Tools}
We consider six static analysis tools for finding bugs in smart contracts in this paper, Oyente, Securify, Mythril, Smartcheck, Manticore, and Slither. %We selected these tools %as they are widely-used, and the papers are highly-cited by researchers. 
They all operate on smart contracts written in Solidity, and are freely available. Further, they are all automated and require no annotations from the programmer.  
We selected Oyente \cite{luu2016making}, Securify \cite{tsankov2018securify}, Mythril \cite{mueller2018smashing}, and Manticore \cite{mossberg2019manticore} as they were used in many smart contract analysis studies \cite{tsankov2018securify, perez2019smart, parizi2018empirical, brent2018vandal}. We included Smartcheck \cite{tikhomirov2018smartcheck} as it uses a pattern matching approach rather than symbolic execution employed by the previous four tools. Similarly Slither \cite{feist2019slither} is another non-symbolic-execution based tool, but unlike SmartCheck, it uses Static Single Assignment (SSA) for analysis.  %and does "deeper" analysis.

%{\bf Oyente}  is a  tool for finding security bugs in smart contracts based on symbolic execution. The EVM bytecode is represented as a Control Flow Graph (CFG). The execution jumps are used as edges that connect the nodes of the graph representing the basic execution blocks in the code. The symbolic execution engine of Oyente uses the CFG and produces a set of symbolic traces, each associated with a path constraint and auxiliary data, to verify pre-defined properties. Oyente works on detecting four types of bugs; namely, transaction order dependency (TOD), unhandled exceptions, timestamp dependencies, and reentrancy. 
%However, it cannot map back the result of the analysis to the function in the code. 

%{\bf SECURIFY} also uses symbolic analysis to analyze both Solidity source code and EVM bytecode. In SECURIFY, each security property is mirrored by defining two kinds of patterns, a compliance pattern that satisfies the property, and a violation pattern that implies its negation. SECURIFY first extracts precise semantic information by symbolically analyzing the dependency graph of the smart contract code. Then it verifies the semantic facts using the already defined patterns of security properties. SECURIFY reduces the effort required to inspect the analysis report, compared to other symbolic analyzers for smart contracts, by classifying behaviors of the analyzed contract into compliant (matched by the compliance patterns), violations (matched by the violation patterns), and warnings (matched by neither).

%{\bf Mythril} is an Ethereum smart contracts security analysis tool with a symbolic execution engine Laser-EVM \cite{laserethereum}. Mythril employs both taint and concolic analysis along with control flow checking to detect a number of security vulnerabilities using an intermediate representation generated from the symbolic traces. %As Oyent, it endures similar incompleteness issues. Mythril can detect a wide range of vulnerabilities that are missed by both Oyente and Securify.

%Similar to Oyente and  Mythril, {\bf Manticore} also employs symbolic execution to detect bugs by extracting execution paths that satisfy a specific property. Unlike the above tools, Manticore can be used for analysis of both Linux ELF binaries and  smart contracts (EVM bytecode).

%Unlike the previous four tools that employ symbolic execution, {\bf SmartCheck} classifies issues by running lexical and syntactical analysis on Solidity source code. 
%SmartCheck translates the source code into an intermediate representation (ID) in the form of XML parse tree using ANTLR \cite{ANTLR} and a custom Solidity grammar. XPath queries on the IR are used to detect the vulnerability patterns.


==> SolidiFI-arXiv (2)/conclusion.tex <==
\pdfoutput=1

\section{Conclusion}
\label{sec:conclu}
This paper proposed \sysname, a technique for performing systematic evaluation of Ethereum smart contract's static analysis tools based on bug injection. \sysname analyzes the AST (Abstract Syntax Tree) of smart-contracts and injects pre-defined bug patterns at all possible locations in the AST.
\sysname was used to evaluate 6 smart contract static analysis tools, and the evaluation results show several cases of bugs that were not detected by the evaluated tools even though those undetected bugs are within the detection scope of tools. \sysname thus identifies important gaps in current static analysis tools for smart contracts, and provides a reproducible set of tests for developers of future static analysis tools. It also allows smart contract developers to understand the limitations of existing static analysis tools with respect to detecting security bugs. 

Future work will consist of expanding \sysname to other smart contract languages than Solidity, and automating the bug definition processes for injecting new bug types. 

==> SolidiFI-arXiv (2)/discussion.tex <==
\pdfoutput=1

\section{Discussion}
\label{sec:discussion}

In this section, we examine the reasons for the false negatives of the tools observed in RQ1.
We then examine the implications of the results, and our methodology, on both tool developers and end users.
Finally, we examine some of the limitations of \sysname and threats to validity of our experiments. 

\subsection{Reasons for False-Negatives}

To establish a practical understanding of the presented results and why some bugs were not detected, we will highlight the code snippets for some of the bugs that were not detected, and then discuss the reasons behind them. We organize this discussion by tool.

\textbf{Oyente} was not able to detect many instances of injected re-entrnacy, timestamp dependency, unhandled exceptions, integer overflow/underflow, and TOD bugs as mentioned earlier
\footnote{Because the released version of Oyente did not work with the latest version of the Solidity compiler (0.5.12), we made few changes to the injected contracts to get it to work with Oyente - these did not impact the tool's coverage.}.
%{\em Oyente} is outdated as it has not been maintained for the last two years and the last version of solidity compiler tested is 0.4.21. We used it in our experiments because  {\em Oyente} is used as a benchmark tool in the field of smart contract security analysis. Since \sysname is using a recent version of solidity compiler (0.5.11), we did slight changes to the injected contracts to be compiled and analyzed correctly with the latest version of {\em Oyente}. Those changes did not impact neither the semantic of the buggy contracts nor their structure (we did not remove or add any instruction), so we were able to inspect the generated analysis reports by {\em Oyente} based on the bug injection logs generated by \sysname. 
According to the paper \cite{luu2016making}, {\em Oyente} works on detecting only re-entrancy bugs that are based on the use of {\em call.value}. Some of the recent tools, such as {\em Slither}, consider the detection of re-entrancy bugs with limited gas that are based on {\em send} and {\em transfer}. Those papers claim that {\em send} and {\em transfer} do not protect from re-entrancy bugs in case of gas price change. Furthermore, {\em Oyente} failed to detect instances of re-entrancy bugs that are based on the use of {\em call.value}.
One of the TOD code snippets we used in our experiments is mentioned in the running example at Figure~\ref{fig:example-contract} on lines 9-16, which emulates a simple game and its winner.  The malicious behavior occurs when the two transactions are executed in one block and the attacker tries to change the order of the received transactions. To understand why this bug is not detected by Oyente, in Oyente the EVM bytecode is represented as a control flow graph (CFG). The execution jumps are used as edges that connect the nodes of the graph representing the basic execution blocks in the code. The symbolic execution engine of Oyente uses the CFG to produce a set of symbolic traces (execution paths), each associated with a path constraint and auxiliary data, to verify pre-defined properties (security bugs being detected). Basically, Oyente detects TOD by comparing the different execution paths and the corresponding data flow (Ether flow) for each path. Oyente reports those different execution paths that have different Ether flows. 

For Oyente to be able to detect all TOD bugs successfully, the symbolic execution engine should generate all possible execution paths for the contract to find the erroneous path  - this is challenging due to the incompleteness of symbolic execution. %In general, {\em Oyente} is neither sound nor complete because it is not able to build a complete control flow graph of the smart contracts. 
It also uses some bounds that limit the symbolic execution.
%so that the path with different Ether flow from others can be found. %especially in this case, where each function is defined as a stand-alone execution block and no common data flow connects both of them.

{\bf Smartcheck} failed to detect most of the injected bugs across all the categories. Smartcheck checks for bugs by constructing an Intermediate Representation (IR) from the source code, and then using XPath patterns to search for bugs in the IR. This approach lacks accuracy as some bugs cannot be expressed as XPath expressions. For example, the re-entracy bug is difficult to express as an XPath pattern, and is hence not detected.
 % (Figure~\ref{fig:re-entrancy}). {\em Smartcheck} did not correctly report any of re-entrancy injected bugs (despite its claim of being able to do so \cite{tikhomirov2018smartcheck}). 
%It misclassfied 1237 out of 1343 injected re-entrancy bugs and did not detect the rest (106 injected bugs). Our use of {\em Smartcheck}, in our experiments, to detect re-entrancy bugs is based on the claim of the tool paper \cite{tikhomirov2018smartcheck} of its ability to detect this type of bugs.

%\begin{figure}[h]
%\centering
%\footnotesize
%\begin{lstlisting}[language= Solidity, basicstyle=\ttfamily]
%function buyTicket() public{
%    lastPlayer.send(jackpot);
%    lastPlayer = msg.sender;
%    jackpot    = this.balance;}
%\end{lstlisting}
%\caption{Re-entrancy code snippet.}
%\label{fig:re-entrancy}
%\end{figure}

%The difficulty of expressing some bugs as XPath patterns is not the only limitation of Smartcheck, 
Further, because Smartcheck uses XPath patterns that detect specific syntax of some bugs,  even a slight variation in the syntax of the bug snippets would not match the XPath patterns. For instance, SmartCheck did not report some occurrences of unhandled exceptions.
% and the reason they were undetected is that that they do not match the exact XPath pattern used to detect timestamp dependency bugs (Section~\ref{sec:vulnerabilities}). 
By checking the code snippet for one of the undetected unhandled exception bug depicted in Figure~\ref{fig:mishandledexp1},
we found that Smartcheck was not able to detect it as unchecked send because Smartcheck only looks for {\em send} functions without an if-statement (that checks the return value). However, in this snippet, the send is within an if-statement even though the {\em revert()} exists in the else clause of the if-statement, which will be triggered on the successes of send. The same happens when other functions are used for sending ether  (e.g., call, etc.) instead of {\em send}. This is an inherent problem with syntactic, rule-based tools such as Smartcheck.
%This weakness can be addressed by checking for proper handling of exceptions instead of looking for {\em send()} that does not fall within the condition of if-statement.
%the send occurs in an if-statement to handle exceptions, and it did not match the syntactic rule used by it even though the revert happens on successful sends (not on failed sends as it should be). 
%  However, Smartcheck was unable to detect that the condition is reversed by the {\em not} operator
 %, and prevent unwanted behaviors. However, Smartcheck was unable to detect that the condition is reversed by the {\em not} operator. 


 \begin{figure}[h]
\centering
\footnotesize
\begin{lstlisting}[language= Solidity, basicstyle=\ttfamily]
if (!addr.send (42 ether))
     {receivers +=1;}
else
     {revert();}}
\end{lstlisting}
\caption{Unhandled exception code snippet 1.}
\label{fig:mishandledexp1}
%\vspace{-4mm}
\end{figure}

{\bf Mythril} was the tool with the largest set of undetected bugs in our experiments. It failed to detect many instances of re-entrancy, timestamp dependency, unchecked send, unhandled exceptions, integer overflow/underflow  and use of tx.origin. For example, the buggy code in Figure~\ref{fig:mishandledexp2} was not detected by Mythril. The condition of the if-statement that checks the return value of the send will always be evaluated as true because of the added condition \enquote{$||$ 1==1}. Hence, the execution of the contract would be reverted in all cases by the function {\em revert()}, regardless of whether the send succeeds. {\em This is incorrect as the execution should only be reverted on the fails of send.} However, Mythril does not detect this as it only evaluates the {\em send()} part in the condition of the if-statement rather than evaluating the whole condition with the OR part ($||$ 1==1).
%as it checks for execution paths that would lead to revert on fails of send regardless of checking if the reverts in those paths are performed only on fails of send rather on both succeeds and fails of send.

{\em Mythril} is also very slow in term of the time it takes to analyze contracts. 
Although we set the time-out for analyzing each contract to 15 minutes, as mentioned earlier, we also tried setting the timeout to 30 minutes and did not observe 
any increase in the number of bugs demonstrating that increasing the time-out has diminishing returns. 
%For example, the number of undetected timestamp bugs decreased from 917 to 810 and from 825 to 755 for uhhandled exception bugs. 
We also found the number of undetected bugs increase in the large contracts, as Mythril enumerates symbolic traces and this does not scale well in large contracts. 
%, as the number of symbolic traces increase in such contracts. 

\begin{figure}[h]
\centering
\footnotesize
\begin{lstlisting}[language= Solidity, basicstyle=\ttfamily]
if (!addr.send (10 ether) || 1==1)
     {revert();}
\end{lstlisting}
\caption{Unhandled exception code snippet 2.}
\label{fig:mishandledexp2}
%\vspace{-4mm}
\end{figure}

Like the other tools, Mythril also misreported the types of many of the injected bugs. 
Figure~\ref{fig:buggy_code} shows part of a buggy contract injected using \sysname. The injected contract allows users to manage their tokens and send tokens to each other. We injected a re-entrancy bug using \sysname in the contract at lines 185-188. However, Mythril reported the re-entrancy bug as  "Unchecked Call Return Value" (i.e., Unhandled exception) at line 186. By inspecting this line of code, we can see that the return value of the {\em send} function is checked and the balance is reset to zero on the success of {\em send}, so there is no unhandled exception as reported. %This raises the question of how Mythril detects unhandled exception bugs, and 
This calls into question Mythril's soundness in detecting this type of bugs as well as its completeness in detecting Re-entrancy bugs.

\begin{figure}[h]
\centering
\footnotesize
\begin{lstlisting}[language= Solidity, basicstyle=\ttfamily, firstnumber=177]
function transfer(address _to, uint256 _value) public returns (bool success) {
    require(balances[msg.sender] >= _value);
    balances[msg.sender] -= _value;
    balances[_to] += _value;
    emit Transfer(msg.sender, _to, _value); 
    return true;
    }
    
function withdraw_balances_re_ent36 () public {
   if (msg.sender.send(balances[msg.sender ]))
        balances[msg.sender] = 0;
      }
\end{lstlisting}
\caption{Part of a buggy contract injected by reentrancy bug.}
\label{fig:buggy_code}
\end{figure}


%\begin{figure}[h] 
%	\centering
%	\includegraphics[width=\columnwidth]{figures/bugLog.PNG}
%	\caption{BugLog generated by \sysname.}
%	\label{fig:buglog}
%\end{figure}

%\begin{figure}[h] 
%	\centering
%	\includegraphics[width=\columnwidth]{figures/mythril_report.PNG}
%	\caption{Mythril analysis report.}
%	\label{fig:mythril_report}
%\end{figure}


{\bf Manticore} was not able to detect instances of re-entrancy and integer overflow/underflow. Unlike other evaluated tools employing symbolic executions, we noticed that Manticore takes a long time to analyze smart contracts, and in some cases it times-out. 
It consumes significant memory space as well on our system. % and some of the tool options (parameters), such as \enquote{core.timeout}, do not work as expected. 
Moreover, Manticore crashed and failed to analyze most of the contracts and threw exception errors. The 50 main contracts  used in our experiments consist of 123 analyzable contracts (each contract file may contain more than one contract). Out of them, {\em Manticore} crashed for 83 contracts injected by re-entrancy bugs and 73 contracts injected by integer overflow bugs. % \asem{Just to clarify, the other tools perform analysis for the whole file while manticore you need to specify the file name and the contract name if the file contains more than on contract}. 
 We reached out to the tool developers to get fixes or explanation for these issues; however, there was no response (as of the time of submission). 
%\karthik{This is good, but why didn't we do this for the other tools.}
%\asem {In the case of Securify, the tool itself did not crash and only gave a message that it failed to analyze contract which is a known case with some tools. But for manticore the tool code itself crash}
%Although this is a long time and might not be practical when used by developers in real-world scenarios, we decided to use this time limit to be conservative. 
%When using Manticore with a source file involving more than a contract, we need to specify which contract to analyze. This questions Manticore scalability and capability of analyzing contracts with code imported from other contracts.  %grant Manticore enough time to analyze contracts and to avoid the cases of not reporting bugs because of the short analysis time.

{\bf Securify} was not able to detect several cases of injected bugs belonging to re-entrancy, unchecked send, unhandled exceptions, and TOD. In addition, we found many cases where {\em Securify} failed to analyze the injected contracts and threw an error.
Out of the 200 contracts injected by the four bug types (50 contracts for each bug type), {\em Securify} failed to analyze 5 contracts injected by unhandled exceptions, 4 injected by re-entrancy, 4 injected by unchecked send, and 4 injected by TOD bugs. If we excluded the injected bugs in those contracts, the number of undetected bugs by {\em Securify} will be as following: (re-entrancy: 105, unchecked send: 332, unhandled exceptions: 402, and TOD: 136). 
{\em Securify} also reported a high number of TOD false positives compared with {\em Oyente}.  A recent study \cite{Feng2019smartscopy} found that the reported false alarms by Securify are due to over-approximation of the execution. % In general, high number of false positives increases the overhead on smart contract developers to find real bugs, and often discourages them from using the tool \cite{Johnson2013}.

{\bf Slither} Although {\em Slither} has almost 100\% accuracy in detecting re-entrancy, timestamp, and tx.origin bugs, it was not able  to detect many instances of unhandled exceptions. Moreover, it had high number of re-entrancy false positives as mentioned earlier. % even though  accuracy in detecting most of the injected bugs. 

\subsection{Implications}
\textbf{Tool Developers}
There are two implications for tool developers. The first implication is that using pattern matching for detecting bugs, especially by employing simple approaches such as XPaths matching, is not an effective way for detecting smart contract bugs for the reasons mentioned earlier in this section. The second point is that bug detection approaches that are based on enumerating symbolic traces are impeded by path explosion and scalability issues. 
%These issues are associated with the use of symbolic execution to find bugs, without employing any solution for path explosion and scalability issues, and more advanced solutions are needed to resolve these issues. 
Therefore, there is a need for sophisticated analysis tools that also consider the semantics of the analyzed code instead of depending only on analyzing the syntax and symbolic traces. For example, static analysis might work better if combined with formal methods that consider the semantic specifications of Solidity and EVM. Recent papers \cite{grishchenko2018semantic, hildenbrandt2017kevm, hirai2017defining, bhargavan2016formal, amani2018towards} have proposed semi-automated formal verification for performing analysis of smart contracts.

\textbf{End Users of Tools}: For smart contract developers, who are the end users of the static analysis tools, there are three implications.
First, they can use \sysname to assess the efficacy of static analysis tools to choose the most reliable tools with no or low false negatives for their use cases. Second, developers should not rely exclusively on static analysis tools, and should test the developed contracts extensively. \sysname can help them build test suites by introducing mutations and checking if the test cases can catch them. Finally, the generated bugs by \sysname and their relative locations in the code can be used for educating developers on writing secure code.

\subsection{Limitations of \sysname}

There are two limitations of \sysname. First, the current version of \sysname works only on Solidity static analysis tools. Although Solidity is the most common language for writing Ethereum smart contracts and most of the proposed tools target analysis of Solidity contracts, \sysname functionality can be easily extended to other languages. %Secondly, \sysname only partially automates the inspection of the tool results and manual inspection is still required to disambiguate some cases.
Secondly, the bug injection approach employed by \sysname requires pre-prepared code snippets (for each bug type), which requires some manual effort. However, this is a one-time cost for each bug type (we have provided these as part of the tool).  
 %Addressing these limitations will be considered in future work. 
 
 \subsection{Threats to Validity}
 
 An external threat to the validity is the limited number of smart contracts considered, namely 50. We have mitigated this threat by considering a wide-range of smart contracts with varying functionality and code sizes.  We emphasize that SolidiFI covers all syntactic elements of Solidity up to version 0.5.12 and, our data-set contains a wide variety of contracts with different features (e.g., loops). Also, we  selected contracts with different sizes that were representative of EtherScan contracts ranging from 39 to 741 locs, with an average of 242 loc (Table~\ref{tab:benchmark}).  
 
 There are two internal threats to validity. First, the number of tools considered is limited to 6. However, as mentioned, these represent the common tools used in other studies on smart contract static analysis. Further, they are widely used in both academia and industry. All the tools available are open-source and are being actively maintained (with the exception of Oyente). Further, the implemented prototype of \sysname is reusable and can be easily extended to evaluate other tools. The second internal threat to validity is that we only injected 7 bug types. However, these bug types have been (1) considered by most of the tools evaluated, and (2) exploited in the past by real attacks. Therefore, we believe they are representative of security bugs in smart contracts.
 
 Finally, a construct threat to validity is our measurement of false-negatives and false-positives. For false-negatives, it is possible that the bugs cannot be exploited in practice. We have partially mitigated this threat by sampling the set of false-negatives and attempting to exploit them (RQ3). For false-positives, it is possible that the reported bugs are true positives. Again, we have partially mitigated this threat by conservatively considering the bugs reported by the majority of the tools for each bug category as true positives. 


==> SolidiFI-arXiv (2)/evaluation.tex <==
\pdfoutput=1

\section{Evaluation} 
\label{sec:eva}
The aim of our evaluation is to measure the efficacy of \sysname in evaluating smart contract static analysis tools, and finding cases of undetected bugs (i.e., false negatives) and false positives. We also measure the performance of \sysname itself, as well as the ability to exploit the undetected bugs. We made all the experimental artifacts used in this study and our results publicly available\footnote{ \url{https://github.com/DependableSystemsLab/SolidiFI-benchmark}}. Our evaluation experiments are thus derived to answer the following research questions:

\begin{itemize}
%\subsection*{\textbf{RQ1} How many potential locations in the code can \sysname inject bugs into compared to the actual ones?}
\item {\textbf{ RQ1.} \it What are the false negatives of the tools being evaluated?}
\item {\textbf{ RQ2.} \it What are the false positives of the tools being evaluated?}
\item {\textbf{RQ3.} \it Can the injected bugs in the contracts be activated (i.e., exploited) at runtime by an external attacker?}
\item {\textbf{RQ4.} \it What is the performance of \sysname?}
\end{itemize}

%The study of the false negatives for static analysis tools might not be enough to evaluate their efficacy.  A tool could look practically efficient simply by reporting the injected bugs; however, it may report several other vulnerabilities that are not real bugs (i.e., false positives). Therefore, we decided to study the false positives of the tools being evaluated along with the study of the false negatives to be able to understand how practically useful each tool is.

As mentioned earlier, we have selected six static analysis tools for evaluation, Oyente \cite{luu2016making}, Securify \cite{tsankov2018securify}, SmartCheck \cite{tikhomirov2018smartcheck}, Mythril \cite{mueller2018smashing}, Manticore \cite{mossberg2019manticore}, and Slither \cite{feist2019slither}. We downloaded these tools from their respective online repositories, which are mentioned in the corresponding papers (Oyente 0.2.7, Securify v1.0 as downloaded and installed in Dec 2019, Mythril 0.21.20,  Smartcheck 2.0, Manticore 0.3.2.1, and Slither 0.6.9).

To perform our experiments, we used a data set of fifty smart contracts, chosen from the list of verified smart contracts available on \textit{Etherscan} \cite{etherscan}, a public repository of smart contracts written in Solidity for Ethereum. We selected these contracts based on three factors namely (1) code size (we selected contracts with different sizes that were representative of Etherscan contracts ranging from small contracts with tens of lines of code to large contracts with hundreds of lines of code), (2) compatibility with Solidity version 0.5.12 (at the time of writing, {\em 312 out of 500 verified smart contracts} in EtherScan supported Solidity 0.5x and higher), and (3) contracts with a wide range of functionality (e.g., tokens, wallets, games). 
%Further, we selected contracts with different sizes that were representative of Etherscan contracts ranging from 39 to 741 locs. 
Table \ref{tab:benchmark} shows the number of lines of code (including comments), and number of functions and function modifiers\footnote{Function modifier checks a condition before the execution of the function.} for each contract. The contracts range from 39 to 741 lines of code (loc), with an average of 242 loc.

 We limited ourselves to 50 contracts due to the time and effort needed to analyze the contracts by the evaluated tools and inspect the analysis results of the tools to verify false-positives. {\em With that said, even with this dataset, SolidiFI found significant numbers of undetected bugs in the tools (e.g., false negatives), as will be discussed in the following sections.} 

As explained in Section \ref{sec:SolidiFI}, in our experiments, we injected bugs belonging to seven different bug types within the detection scope of the selected tools. Table \ref{tab:bugsandtools} shows the bug types, and the tools that are designed to detect each bug type. We chose these bug types based on the bug types detected by the individual tools, and because these bugs are common in smart contracts, and lead to vulnerabilities that have been exploited in practice~\cite{dao2017,batchOverflow, EthereumAttacksHistory}. However, \sysname is not confined to these bug types. 

In our experiments, we set the time-out value for each tool to 15 minutes per smart contract and bug type. If a tool's execution exceeds this timeout value, 
we terminate it and consider the bugs found as its output. While 15 minutes may seem high, our goal is to give each tool as much leeway as possible.
Only 2 of the tools exceeded this time limit in some cases (i.e., Mythril and Manticore). For these two tools, we experimented with larger timeout values, 
but they did not significantly increase their detection coverage. Note that the total time taken to run the experiments was already quite high with this
timeout value - for example, it took us about 4 days to analyze the contracts using Mythril (50-contract*6 bug-types*15-minute = 75 hours). 

\begin{table}[h]
\begin{center}
\caption{Contracts benchmark. F represents Functions, and M represents Function Modifiers}
\begin{tabular}{|c|c|c||c|c|c||c|c|c|}  
\hline
 \textbf{Id}&{\rotatebox{90}{\textbf{Lines}}}&{\rotatebox{90}{\textbf{F+M}}}& \textbf{Id}&{\rotatebox{90}{\textbf{Lines}}}&{\rotatebox{90}{\textbf{F+M}}}& \textbf{Id}&{\rotatebox{90}{\textbf{Lines}}}&{\rotatebox{90}{\textbf{F+M}}} \\
\hline
1&103&6&18&406&29&35&317&29\\
\hline
2&128&9&19&218&32&36&383&20\\
\hline
3&132&10&20&308&27&37&368&24\\
\hline
4&117&6&21&353&18&38&195&24\\
\hline
5&250&17&22&383&19&39&52&4\\
\hline
6&161&22&23&308&20&40&465&22\\
\hline
7&165&22&24&741&27&41&160&8\\
\hline
8&251&17&25&196&12&42&128&16\\
\hline
9&249&19&26&143&20&43&285&22\\
\hline
10&39&5&27&336&33&44&298&24\\
\hline
11&193&19&28&195&24&45&156&14\\
\hline
12&281&27&29&312&13&46&125&6\\
\hline
13&161&8&30&711&57&47&223&18\\
\hline
14&185&20&31&216&12&48&232&19\\
\hline
15&160&8&32&143&14&49&52&4\\
\hline
16&248&27&33&129&16&50&171&18\\
\hline
17&128&17&34&445&29&&&\\
\hline
\multicolumn{7}{|c|}{\textbf{Average values }}&\textbf{242}&\textbf{18}\\
\hline
\end{tabular}
\label{tab:benchmark}
\end{center}
%\vspace{-7mm}
\end{table}

\begin{table}[h]
\begin{center}
\caption{Bug types used in our evaluation experiments: '*' means that the tool can detect the bug type.}
\begin{tabular}{|c|c|c|c|c|c|c|}  
\hline
 \textbf{Bug Type}&{\rotatebox{90}{\textbf{Oyente}}}&{\rotatebox{90}{\textbf{Securify}}}&{\rotatebox{90}{\textbf{Mythril}}}&{\rotatebox{90}{\textbf{SmartCheck}}}&{\rotatebox{90}{\textbf{Manticore}}}&{\rotatebox{90}{\textbf{Slither}}} \\
 \hline
 Re-entrancy &* & * & * & *&* &*\\
\hline
%Missing constructor & & & * & \\
%\hline
Timestamp dependency &* & & * & *&&* \\
\hline
Unchecked send & & * & * & &&\\
\hline
Unhandled exceptions &* & * & * & *&&* \\
\hline
TOD&* & *& & &&\\
\hline
Integer overflow/underflow & *& & * & *&* &\\
\hline
Use of tx.origin & & & * & * &&*\\
\hline
%DoS by external contract & & & * & * &&\\
%\hline
\end{tabular}
\label{tab:bugsandtools}
\end{center}
%\vspace{-7mm}
\end{table}

\smallskip \subsection{RQ1:What are the false negatives of the tools being evaluated?}

The core part of our evaluation is to use \sysname to inject bugs, and evaluate the effectiveness of the tools in detecting the injected bugs. 
We performed the following steps in our experiments. First, \sysname is used to inject bugs of each bug type in the code of the 50 smart contracts, one bug type at a time. % at all possible locations, one at a time. 
The resulting buggy contracts are then checked using the static analysis tools. %We also check that the bugs do not cause the contract to mis-compile. 
Finally, %we perform a combination of automated and manual inspection of the tool results for each contract, and 
the number of the injected bugs that were not detected by each tool were recorded. % as undetected bugs. 

%This process is repeated for all the bug types. 

To get meaningful results, we inject bugs that are as distinct as possible by preparing diverse set of distinct code snippets with different data inputs and function calls- this resulted in $9369$ distinct bugs.
We consider two injected bugs as distinct if the static analysis tool under study would reason about them differently based on the underlying methodology, where either the data and control flow leading to the injected bug is different, or the design patterns of the bug snippets are different. 
{\em To  ensure a fair evaluation, we inject only the bugs that are supposed to be detected by each tool. }% - otherwise, we do not count the tool's failure to detect it as a false negative.} 

We consider an injected bug as being correctly detected by a tool if and only if it identified both the line of code in which the bug was injected, as well as the bug type (e.g., Re-entrancy). 
In many cases, we observed that the tool would correctly identify the line of code in which the bug occurred, but would misidentify the bug type. Therefore,
we also report the former separately.
%We consider these as incorrect detections, but also report the former separately. 

The results of injecting bugs of each bug type, and testing them using the six tools are summarized in Table \ref{tab:flasenegative}. 
%For simplicity, this table shows the overall results of undetected bugs for each tool.
 In the table, \enquote{Injected bugs} column specifies the total number of injected bug for each bug type, \enquote{\checkmark}  means we did not find any undetected bug of that bug type (row), while \enquote{NA} means the bug type is out of scope of the tool, i.e., it is not designed to detect the bug type. The numbers for each column specify the total number of bugs that were either incorrectly detected or not detected by the tool corresponding to the bug type specified in that row.
 The number within parentheses specifies the number of cases that were not reported by the tool - this does not consider the incorrect reporting of the bug type.%the reported line number was correct, but the reported bug type was incorrect (i.e., misclassification). 
% \karthik{What about cases where the tool timed out?} \asem{I was thinking to comment on this in the discussion section }
 
 %By inspecting the false negatives of the tools, we found that the tool either was not able to detect a bug or the tool wrongly reported the bug as another bug type (misclassification). Therefore, the table shows two numbers for each bug type. The number on the top states the total number of undetected and misclassified bugs while the number between the brackets states the total number of misclassified bugs. 
 
 From the table, we can see that a significant number of false negatives occur for all the evaluated tools,
 and that {\em none of the tools was able to detect all the injected bugs correctly even if we accepted a incorrect bug type with the correct line number as a detected bug}.
 In fact, the only tool that had 100\% coverage for individual bug types was Slither, for {\em Reentrancy} and {\em tx.origin} bugs.
 Of all tools, Slither had the lowest false-negatives, followed by Securify across bug types.
  %However, if we checked the results based on the bug type level, {\em Slither} had 100\% accuracy in detecting Re-entrancy bugs.
 %However, if we are prepared to accept a misclassified bug type with the correct line number as a detected bug, then {\em Slither} had 100\% accuracy in detecting bugs, and {\em Securify} came second.  
% The only tool that detected all the injected bugs while wrongly classified some of them  was {\it Slither}, and it is the only tool that successfully detected all Re-entrancy bugs. 

% {\em Even with the adopted technique for injecting bugs (that can be considered as simple), we found many instances where static analysis tools do not find the injected bugs, thus showing the efficacy of our technique. In addition, the simplicity of the injected bugs doubts the sophistication
Our results thus show that all static analysis tools have many corner cases of bugs that they are not able to detect.
{\em Note that it is surprising that our technique found as many undetected bugs by the tools as it did, given that our goal was not specifically to exercise corner cases of the tools in question.} 
%{\em The relatively large number of undetected bugs also reveal flaws in the designs of the evaluated tools rather than just implementation issues}. 
We will discuss the reasons for the missed detections and the implications later (Section~\ref{sec:discussion}).

\begin{table}[h]\footnotesize
\begin{center}
\caption{False negatives for each tool. Numbers within parantheses are bugs with incorrect line numbers or unreported.}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
 \textbf{Security bug} &{\rotatebox{90}{\textbf{Injected bugs}}}&{\rotatebox{90}{\textbf{Oyente}}} &{\rotatebox{90}{\textbf{Securify}}}&{\rotatebox{90}{\textbf{Mythril}}}&{\rotatebox{90}{\textbf{SmartCheck}}}&{\rotatebox{90}{\textbf{Manticore}}}&
 {\rotatebox{90}{\textbf{Slither}}}\\
 \hline
 Re-entrancy&1343 &\shortstack{1008 \\ (844)}&\shortstack{232\\(232)}&\shortstack{1085\\(805)}& \shortstack{1343\\(106)}&\shortstack{1250\\(1108)}&\cellcolor{asparagus}\checkmark\\
\hline
%Missing constructor &--&--&--&--\\
%\hline
Timestamp dep&1381 &\shortstack{1381\\(886)}&\cellcolor{lightgray}NA&\shortstack{810\\(810)}& \shortstack{902\\(341)}&\cellcolor{lightgray}NA&\shortstack{537\\(1)} \\
\hline
Unchecked-send&1266 &\cellcolor{lightgray}NA&\shortstack{499\\(449)}& \shortstack{389\\(389)} & \cellcolor{lightgray}NA&\cellcolor{lightgray}NA &\cellcolor{lightgray}NA\\
\hline
Unhandled exp&1374 &\shortstack{1052\\(918)}
&\shortstack{673\\(571)}& \shortstack{756\\(756)} &\shortstack{1325\\(1170)}&NA&\shortstack{457\\(128)}\\
\hline
TOD &1336& \shortstack{1199\\(1199)} &\shortstack{263\\(263)}&\cellcolor{lightgray}NA&\cellcolor{lightgray}NA&\cellcolor{lightgray}NA&\cellcolor{lightgray}NA\\
\hline
Integer overflow&1333 &\shortstack{898\\(898)}&\cellcolor{lightgray}NA&\shortstack{1069\\(932)}&\shortstack{1072\\(1072)}&\shortstack{1196\\(1127)}&\cellcolor{lightgray}NA\\
\hline
tx.origin &1336&\cellcolor{lightgray}NA&\cellcolor{lightgray}NA&\shortstack{445\\(445)}&\shortstack{1239\\(1120)}&\cellcolor{lightgray}NA&\cellcolor{asparagus}\checkmark\\
\hline
%DoS& 1333 &\cellcolor{lightgray}NA&\cellcolor{lightgray}NA&50& 119&\cellcolor{lightgray}NA &\cellcolor{lightgray}NA\\
%\hline
\end{tabular}
\label{tab:flasenegative}
\end{center}
%\vspace{-4mm}
\end{table}

 \subsection{RQ2: What are the false positives of the tools being evaluated?}
 
%In addition to inspecting the results of each tool for those injected but undetected bugs, we check the other reported bugs to see whether they are real bugs or just false alarms. 
A false-positive occurs when a tool reports a bug, but there was no bug in reality. Unlike false negatives, where we know exactly where the bugs have been injected, and hence have ground truth, measuring false positives is challenging due to the lack of ground truth. 
This is because we cannot assume that the smart contracts used are free of bugs (though they are chosen from the verified contracts on Etherscan). 
Further, manually inspecting each bug report and related contract involves a tremendous amount of effort due to the large number of bug reports, and is hence not practical.

To keep the problem of determining false-positives tractable, we came up with the following approach.
The main idea is to manually examine only those bugs that are {\em not} reported by the majority of the other tools for each smart contract. In other words, we
conservatively assume that a bug that is reported by a majority of the tools cannot be a false positive. However, at worst, we will underestimate
the number of false positives in this approach, subject to the vagaries of the manual inspection process. We also verified that many of the bugs
that are excluded by the majority are indeed false-positives by manually examining a random sample of them.
 
Even after this filtering, we had to manually inspect a significant
number of bugs to determine if they were false positives. Therefore, for each tool, we randomly selected 20 bugs of each bug type category that were not excluded by the majority approach, and inspected them manually. For those cases where the number of bugs is less than or equal to 20, we inspected them all. %This resulted in inspecting about $202$ bugs manually.
Based on the results of our manual inspection, we estimated the false positives as the percentage of bugs inspected that were indeed false positives, multiplied by the number of bugs filtered (i.e., not excluded).

For example, assume that the total number of bugs reported by a tool is $100$. Of these 100 bugs, let us assume that $60$ are also reported by the majority of the other tools for the smart contract, and hence we exclude them. Of the remaining $40$ filtered bugs, we manually examine $20$ bugs chosen at random. Assume that $16$ of these are indeed false-positives. 
We assume that 80\% of the filtered bugs are false-positives, and estimate the number of false-positives to be $32$. 
%While there is some inaccuracy in this approach, we believe it provides a balance between effort and accuracy. 
%While we acknowledge the limitations of this approach, we are unable to come up with a more robust approach for finding false-positives that does not require significant manual effort.

%We found that most such bugs were indeed true false-positives.
 
The results of false positives reported by each tool are summarized in Table \ref{tab:flasepositive}. In the table, the \enquote{Threshold} column refers to the majority threshold, which is the number of tools that must detect the bug in order for it to be excluded from consideration - this number depends on how many tools are able to detect the bug type. 
%As before, \enquote{NA} means the bug type is out of scope of the tool.
For each tool, the sub-column \enquote{Reported} shows the number of bugs reported by the tool, 
the sub column \enquote{FIL} shows the number of bugs that have been filtered (not excluded) by the majority approach,
 while the sub column \enquote{FP} shows the false positives of the tool based on the manual inspection as explained above. 
 Empty cells in the table represent cases where a tool was not designed to detect a bug type. 
 Note that some of the tools detected bugs outside the 7 categories that we considered - we called these as {\em miscellaneous}.
% Since in our experiments we are more focused on bugs belonging to 7 categories (most of them have real-world exploit incidents), some of the tools work on detecting other bug types. Therefore, we have put the reported bugs outside the scope of the 7 bug types under the \enquote{miscellaneous} category.

From the table, we can see that all the evaluated tools have reported a number of false positives, ranging from $2$ to $801$ for most of the bug types.
Interestingly, the results show that the tools with low numbers of false negatives reported high false positives, i.e., {\em Slither} and {\em Securify}. 
For example, although {\em Slither} was the only tool that successfully detected all the injected Re-entrancy bugs, it reported significant false positives.
This raises the question of whether the high detection rate was simply a result of over-zealously reporting bugs by the tool (this is
also borne out by the high number of bugs reported under the {\em miscellaneous} category by this tool).
%, especially with the consideration of the large number of bugs reported by  this tool which involves about $2262$ bugs under the miscellaneous category. 
{\em  This highlights the need for security analysis tools that are able to detect bugs while maintaining low false positive rates.}
 
We provide some examples of the false-positive cases below. 
For example, most unhandled exception bugs were reported even though the code checks the return values of the send functions for exceptions using {\em require()}. As another example, many false positives were re-entrancy bugs where the code contains the required checks of the contract balance, and updates the contract states before the Ether transfer. Oyente reported several cases as integer over/underflow even though they are no integer related calculations (e.g., {\em string public symbol = "CRE";}). On the other side, we tried to be consistent with the assumptions considered by the tools during our manual inspection. For example, some of the cases that we considered as true bugs were re-entrancy bugs  that use the {\em transfer} function. This function protects against re-entrancy issues as it has limited gas; however, we considered them as true bugs as the attack can happen if the gas price changes - this is detected by some of the tools (e.g., Slither).

\begin{table*}[h]\footnotesize
\begin{center}
\caption{False positives reported by each tool. Empty cells mean that the tool was not designed for that particular bug type.}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}  
\hline
 \textbf{Bug Type}&{\rotatebox{90}{\textbf{Threshold}}}&\multicolumn{3}{|c|}{\rotatebox{90}{\textbf{Oyente}}}&\multicolumn{3}{|c|}{\rotatebox{90}{\textbf{Securify}}}&\multicolumn{3}{|c|}{\rotatebox{90}{\textbf{Mythril}}}&\multicolumn{3}{|c|}{\rotatebox{90}{\textbf{SmartCheck}}}&\multicolumn{3}{|c|}{\rotatebox{90}{\textbf{Manticore}}}&\multicolumn{3}{|c|}{\rotatebox{90}{\textbf{Slither}}} \\
 \hline
= &&Reported&FIL&FP&Reported&FIL&FP&Reported&FIL&FP& Reported&FIL&FP&Reported&FIL&FP&Reported&FIL&FP\\
 \hline
 Re-entrancy & 4& 0 &0&- &12 & 12&12&54&54&43&0&0&-&6&6&6&79&79&71\\
\hline
%Missing constructor & & & * & \\
%\hline
Timestamp dep & 3& 0&0 &- & &&& 12&12&0&0&0&-&&&&12&12&0\\
\hline
Unchecked send & 2& &  &&7 &4&4&14&3&3&&&&&&&&&\\
\hline
Unhandled exp & 3&10  &10 & 10 &0&0&-&0&0&-&6&6&6&&&&0&0&- \\
\hline
TOD&2 &32 &24& 24 &121 &97&97&&&&&&&&&&&&\\
\hline
Over/under flow &3 &947 &943 &801 & && &17&3&3&3&2&2&9&9&9&&&\\
\hline
Use of tx.origin &2 & &&  & &&&0&0&-&3&1&0&&&&4&2&0\\
\hline
%DoS & 2& & & &  &&&&&&&&&&&&&&\\
%\hline
Miscellaneous && 0  &&&318&&&144&&&1520&&&169&&&1807&&\\
\hline
\end{tabular}
\label{tab:flasepositive}
\end{center}
%\vspace{-4mm}
\end{table*}

\smallskip \subsection{RQ3: Can the injected bugs be activated by an external attacker?}
%After evaluating the capability of \sysname in injecting bugs into all potential locations in the code, in this section, 
The goal of this RQ is to assess whether the undetected bugs in RQ1 can be activated in the contract at runtime. This is to determine whether the reason behind the bug not being detected by the evaluated tool was because the bug cannot be activated (and hence cannot be exploited by an attacker). We deploy the set of buggy contracts with the undetected bugs (found in RQ1) on the Ethereum blockchain, and execute transactions that attempt to activate them. 

To conduct these experiments, we use MetaMask \cite{MetaMask}, a browser extension that allows us to connect to an Ethereum node called INFURA \cite{INFURA}, and run our buggy contracts on this node. We have created Ethereum accounts on Ethereum Kovan Testnet (test network) using MetaMask, and deposited sufficient amount of Ether to these accounts to enable us to execute transactions (pay the required gas for transactions). We use Remix \cite{remix} (Solidity editor) to deploy contracts on Ethereum Kovan Testnet.  Remix enables us to connect with MetaMask to deploy contracts on INFURA Ethereum node. %To interact with the deployed contracts, we developed a Python client.
% that interacts with Ethereum employing Web3 library. We use this client to create Ethereum transactions, call smart contract functions, and read/write data from/to smart contracts.

%As we are injecting large number of bugs, we will focus our experiments here on interacting with randomly selected samples of those injected bugs that were not detected by the evaluated tools to check their activity in the buggy contracts. We will explain our process with one complete experiment and then discuss the obtained results for the rest of our experiments. 

We illustrate the process with an example. As mentioned in RQ1, Manticore did not report instances of injected integer overflow/underflow bugs - an example is shown in Figure \ref{fig:undetected-underflow}. Our goal is to attempt to activate this bug in the deployed buggy contract by calling the function \textit{bug\_intou3()}. The returned result was 246 - this is not the expected value (-10) due to the use of unsigned integer type (i.e., uint8) instead of a signed integer type, which resulted in an integer underflow. Thus, the bug can be activated by an attacker. 

We had to manually craft inputs for each bug in order to test its activation, which takes significant effort. 
 Because of the large number of undetected bugs, we selected 5 undetected bugs for each bug type randomly from different contracts to test their activation. Table \ref{tab:bugsactivity} shows the results of our activation experiments.  In the table \enquote{--} means we were not able to perform experiments on this bug type, as it requires the attacker to behave as a miner, which would consume a significant amount of computational resources. The results show that one can exploit (activate) all the selected bugs in their related buggy contracts. %This highlights the efficacy of the bug injection approach used by \sysname in injecting activatable bugs in the source code of the contracts. Moreover, the results show that 
 Therefore, the infeasibility of activation of the bug was not the reason that the evaluated tools failed to detect the injected bugs. %was the reason for not detecting those injected active bugs.

\begin{figure}[h]
\footnotesize
\centering
\begin{lstlisting}[basicstyle=\ttfamily]
function bug_intou3() public{
    uint8 vundflw =0;
    vundflw = vundflw -10; // underflow
    return vundflw;}
\end{lstlisting}
\caption{Undetected integer underflow bug}
\label{fig:undetected-underflow}
%\vspace{-8mm}
\end{figure}

%We deployed the related buggy contract containing this bug on Ethereum Kovan Testnet. After that we used our developed Python client to 


\begin{table}[h]
\begin{center}
\caption{Activity of Selected Undetected Bugs. }
\begin{tabular}{|c|c|c|}  
\hline
 \textbf{Bug type}&\textbf{Selected bugs}&\textbf{Activated bugs }\\
 \hline
 Re-entrancy &5 &5  \\
\hline
Timestamp dependency &5 & 5\\
\hline
Unchecked send &5 &5 \\
\hline
Unhandled exceptions &5 &5 \\
\hline
TOD& -- & -- \\
\hline
Integer overflow/underflow &5 &5 \\
\hline
Use of tx.origin &5 &5 \\
\hline
%DoS by external contract &5&5 \\
%\hline
\end{tabular}
\label{tab:bugsactivity}
\end{center}
%\vspace{-6mm}
\end{table}


\smallskip \subsection{RQ4: What is the performance of \sysname?} 
Finally, we measured the performance of \sysname in terms of the time it takes to inject bugs and generate buggy contracts. We excluded the time of running the tools being evaluated to check the buggy contracts, as this is tool-specific and independent of \sysname. 
%Figure %\ref{fig:runtime} shows the time of injecting the eight bug types in each contract, one bug type at a time. 
We preformed injection of each bug type in each contract five times and  calculated the average of the five runs, and then calculated the average of injecting the seven bug types in each contract. The average time of injecting all instances of bug types in a contract is 25 seconds, and the worst case time was 46 seconds (for contract 24, which was the largest contract in our set). {\em Thus, \sysname takes less than 1 minute on average per contract and bug type. } 
% This is redundant - we say it in limitations
%Note that we did not include the time taken for inspecting the results of the tools, as the inspection procedure is only semi-automated, and we perform a combination of manual and automated inspection in our experiments. \karthik{Why did we need to do this?}
%\begin{figure}[h] 
%\centering
%\includegraphics[width=0.95\columnwidth,trim={0 0.5in 0 0},clip]{figures/runtime.eps}
%\caption{\sysname Runtime.}
%\label{fig:runtime}
%\end{figure}
%\begin{table}[h]
%\begin{center}
%\caption{\sysname runtime.}
%\begin{tabular}{|c|c|c|c|c|c|}
%\hline
%Contract&time(sec)&Contract&Time(sec)&Contract&Time(sec)\\
%\hline
%1&51.8&6&79.8&11&103.6\\
%\hline
%2&89.6&7&93.8&12&182\\
%\hline
%3&95.2&8&138.6&13&98\\
%\hline
%4&84&9&113.4&14&128.8\\
%\hline
%5&127.4&10&30.8&15&58.8\\
%\hline
%\multicolumn{2}{|c|}{Average(sec)}&\multicolumn{4}{|c|}{98.4}\\
%\hline
%\end{tabular}
%\label{tab:runtime}
%\end{center}
%\end{table}


==> SolidiFI-arXiv (2)/implementation.tex <==
\pdfoutput=1

\section{\sysname Algorithm} 
\label{imp}
This section explains the  main algorithm of \textit{\sysname}. 
The process of evaluating static analysis tools by injecting bugs in a smart contract source code goes through four steps:
\begin{enumerate}
    \item Compile a version of the target contract and generate the Abstract Syntax Tree (AST).
    \item Use the generated AST to identify the potential locations for injecting bugs and generate an annotated AST marking all identified locations.
    \item Inject bugs into the marked locations to generate the buggy contract.
    \item Check the buggy contract using the evaluated tools and inspect the results for undetected bugs.
\end{enumerate}

The four steps are depicted in Figure \ref{fig:solidifi}, and Algorithm \ref{alg:solidifi} provides a high-level description of \sysname procedure for evaluating static analysis tools.

\begin{figure}[h] 
\centering
\includegraphics[width=0.75\columnwidth]{figures/solidifi.eps}
\caption{\sysname Components}
\label{fig:solidifi}
\end{figure}

\small
\begin{algorithm}[h]
\caption{\sysname High-level Algorithm}
\label{alg:solidifi}
\begin{algorithmic}[1]
\Procedure{main}{}
\State $AST \gets Parser(contract.sol)$
\For{Each bug type}
\State $FIP \gets Find All Potential Locations(AST)$
\For{Each location in FIP}
 \State{Decide injection approach}
 \If{approach  == inject snippet}
    \State{Inject matching bug snippet}
  \ElsIf{approach  == weaken security}
  \State{Weaken existing security mechanism}
  \ElsIf{approach  == transform code}
    \State{Do required code transformation}
  \EndIf
 \State{Record injection details in BugLog}
 \EndFor
 \EndFor
 \For{Each tool being evaluated}
  \State $Result \gets Check(buggyContract)$
  \State $Undetected Bugs \gets Inspect(result)$
 \EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}
\normalsize

\textbf{Abstract syntax tree generation:}
First, \sysname reads the source code of the target contract and compiles it to make sure it is a compiled version. Then abstract syntax tree (AST) of the  target contract is generated (line 1 in Algorithm \ref{alg:solidifi}).

\textbf{Bug locations identification:}
The generated AST is passed to \textit{Bug Locations Identifier}, that drives a bug injection profile (BIP) of all possible injection locations in the target contract for a given security bug (line 4 in Algorithm \ref{alg:solidifi}). FIP is derived using AST-based analysis for identifying potential injection locations in smart contract code. The process of identifying the possible locations for injecting a specific bug in the target contract depends on specific rules that specify the relation between the nature of the bug to be injected and the target contract structure. In general, bugs take two forms: an individual statement and a block of statements. A block of statements can be defined either as a stand-alone function or non-function block such as if statement. Therefore, we use a rule for each form of the bugs that defines the specifications of the locations in which the injection would be possible. For example, the specifications of the locations for injecting a bug formulated as a stand-alone function would be any location that is within the body of the contract and not inside the body of another function or conditional statement. \karthik{Can you show the actual rule - is it written as a grammar?}

\textbf{Bug injection and code transformation:}
\sysname uses a systematic approach toward injecting bugs into the potential locations in the target contract (lines 6-13 in Algorithm \ref{alg:solidifi}). The \textit{AST Transformer} model seeds a bug for each location specified in the FIP. It uses AST-based code transformation to modify the code. 
Three different approaches are used to inject bugs as discussed in Section \ref{buginstrument}.

In addition to injecting bugs in the target contract, \textit{Bug Injector} generates a \textit {BugLog} that specifies a unique identifier for each injected bug, and the corresponding location/s in the target contract where it has been injected (line 14 in Algorithm \ref{alg:solidifi}). The \textit{BugLog} is used for performing automated inspection of the scan results generated by the evaluated tools, to find a list of the injected bugs that were not detected.

\textbf{Buggy code check and results inspection:}
The resulting buggy contract is passed to the \textit{Tool Evaluator} that check the buggy code using the tools under evaluation (line 18 in Algorithm \ref{alg:solidifi}). It then scans the results generated by the tools looking for the bugs that were injected but undetected, with the help of \textit{BugLog} generated by the \textit{Bug Injector} (line 19 in Algorithm \ref{alg:solidifi}). A list of undetected bugs is the output of \sysname.

\section{Implementation}
\sysname uses Solidity compiler \textbf{solc} (mainly version 0.5.8) to compile the original source code file to make sure it is free from compilation errors before it is injected. In addition, \sysname uses \textbf{solc} to generate AST of the original code in json format. We have implemented the other components of \sysname in Python in about 435 lines of code. Those components are responsible for identifying the potential locations for injection, injecting bugs using suitable injection approach, and generating the buggy contract. In addition to implementing the component responsible for inspecting the results of the evaluated tools and then reporting the undetected bugs. 

==> SolidiFI-arXiv (2)/introduction.tex <==
\pdfoutput=1

\section{Introduction}

The past few years have witnessed a dramatic rise in the popularity of smart contracts \cite{clack2016smart}. Smart contracts are small programs written into blocks running on top of a blockchain that can receive and execute transactions autonomously without trusted third parties~\cite{grishchenko2018semantic}.
Ethereum  \cite{buterin2014ethereum} is the most popular framework for executing smart contracts. %Similar to other blockchain systems, Ethereum has the concept of user accounts that are governed by a private-public key pair, which can send transactions between each other. %However, unlike other blockchain systems, Ethereum also has the concept of smart contracts. 

%Serpent, LLL, Mutan, Viper, etc. Solidity is a Turing-complete programming language and the most popular for writing Ethereum contracts. 
%Smart contracts are compiled and deployed as Ethereum virtual machine bytecode. 
%The resulting bytecode is executed on every incoming transaction by distributed nodes, called miners, using the consensus protocol of blockchain in a decentralized manner. 
%Ethereum smart contracts are used in cases such as digital identity, trade finance, financial data recording, intellectual property rights, mortgages, supply chain, crowdfunding schemes, shared wallets, etc.

%As smart contracts are written by fallible human developers,L
Like all software, smart contracts may contain bugs. 
Unfortunately, bugs in smart contracts can be exploited by malicious attackers for financial gains. 
In addition, transactions on Ethereum are immutable and cannot be reverted, so losses cannot be recovered. 
Further, it is difficult to update a smart contract after its deployment. Consequently, there have been many bugs in smart contracts that have been maliciously exploited in the recent past \cite{dao2017, paritywalletbreach2017, mathieu2017blocktix}.
%The last two years witnessed several attacks that exploited code vulnerabilities found in the targeted smart contracts. 
%For example, the DAO vulnerability, led to a \$60 million worth of Ether theft \cite{dao2017}. Another bug in Parity's wallet, a leading Ethereum provider, was exploited by an attacker to steal  \$31 million worth of Ether  \cite{paritywalletbreach2017}. 
%Yet another code vulnerability in a multi-signature wallet enabled an attacker to make herself an owner and lock all the Ether up in the contract \cite{mathieu2017blocktix}. %, effectively mounting a Denial-of-Service  (DoS) attack. 
% Karthik - removed this sentence as we don't deal with fraud in smart contracts
%Further, a recent study \cite{atzei2017survey} found that many fraudulent smart contracts are deployed in the wild. 
%Given the financial importance of smart contracts, and the restriction that they cannot be updated after being deployed on blockchain, security bugs in smart contracts are highly critical. 
Therefore, there is a compelling need to analyze smart contracts to detect and fix security bugs.
%Static  analysis is typically used for this purpose. 
%Statically analyzing smart contracts for vulnerabilities and bugs has become a major research topic in the last three years. 

Several approaches and tools have been developed that statically find security bugs in smart contracts~\cite{luu2016making, mueller2018smashing, tsankov2018securify, tikhomirov2018smartcheck, feist2019slither}. 
However, despite the prevalence of these static analysis tools, security bugs abound in smart contracts~\cite{perez2019smart}. This calls into
question the efficacy of these tools and their associated techniques. Unfortunately, many of the static analysis tools
have been evaluated either only by their developers on custom data-sets and inputs, often in an ad-hoc manner, or on data-sets of contracts with a limited number of bugs (112 bugs \cite{durieux2019empirical} and 10 bugs \cite{parizi2018empirical}). {\em To the best of our knowledge,
there is no systematic method to evaluate static analysis tools for smart contracts regarding their effectiveness in finding security bugs.} 
%most evaluations of the proposed tools have been performed by the tool developers, and we are aware of no comprehensive evaluations. In addition, the evaluations of the proposed tools have been done independently and no systematic approach has been used yet to evaluate existing tools for static analysis of Ethereum smart contracts. 

Typically, static analysis tools can have both false-positives and false-negatives. While false positives are important,  false negatives in smart contracts can lead to critical consequences, as exploiting bugs in contracts usually leads to loss of ether (money). Also, empirical studies of software defects in the field have found that many of the defects can be detected by static analysis tools in theory, but are not detected due to limitations of the tools~\cite{thung2012extent}. 
In our work, we focus mostly on the undetected bugs (i.e., false negatives), though we also study false-positives of the tools.
%false alarms of static analysis tools for smart contracts written in Solidity.%Therefore, we study the undetected bugs of static analysis tools (i.e., false negatives) for smart contracts written in Solidity.

We perform bug injection to evaluate the false-negatives of smart contract static analysis tools. 
Bug injection as a testing approach has been extensively explored in the domain of traditional programs \cite{pewny2016evilcoder,dolan2016lava,bonett2018discovering}; 
however, there have been few papers on bug injection in the context of smart contracts. 
This problem is challenging for two reasons. 
First, smart contracts on Ethereum are written using the Solidity language, which differs from conventional programming languages 
typically targeted by mutation testing tools \cite{dannen2017introducing}.
Second, because our goal is to inject security bugs, the bugs injected should lead to exploitable vulnerabilities. 

%To help developers enhance the developed tools, and researchers in their quest to develop effective static analysis mechanisms of smart contracts, 
This paper proposes \sysname\footnote{\sysname stands for Solidity Fault Injector, pronounced as Solidify. }, a methodology for systematic evaluation of smart contracts' 
static analysis tools to discover potential flaws in the tools that lead to undetected security bugs. 
\sysname injects bugs formulated as code snippets into {\em all} possible locations into a smart contract's source code written in Solidity. 
The code snippets are vulnerable to specific security vulnerabilities that can be exploited by an attacker. 
The resulting buggy smart contracts are then analyzed using the static analysis tools being evaluated, and the results are inspected for those injected bugs that are not detected by each tool - these are the false-negatives of the tool. 
%, and for secure code patterns reported wrongly as bugs - these are the false-positives of the tool. 
Because our methodology is agnostic of the tool being evaluated, it can be applied to any static analysis tool that works on Solidity.  

We make the following contributions in this paper.

\begin{itemize}	
    \item Design a systematic approach for evaluating false-negatives and false-positives of smart contracts' static analysis tools.
    \item Implement our approach as an automated tool, \sysname, to inject security bugs into smart contracts written in Solidity.    
    \item Use \sysname to evaluate six static analysis tools of Ethereum smart contracts for false-negatives and false-positives.
     \item Provide an analysis of the undetected security bugs and false-positives for the 6 tools, and the reasons behind them. 
     \end{itemize}

The results of using \sysname on 50 contracts show that all of the evaluated tools had significant false-negatives ranging from $129$ to $4137$ undetected bugs across 7 different bug types despite their claims of being able to detect such bugs, as well as many false positives. Further, many of the undetected bugs were found to be exploitable when the contract is executed on the blockchain.
Finally, we find that \sysname takes less than 1 minute to inject bugs into a smart contract (on average). 
Our results can be used by tool developers to enhance the evaluated tools, and by researchers proposing new bug-finding tools for smart contracts. 

%The rest of this paper is organized as follows. Section \ref{sec:background} provides an overview of Ethereum smart contracts and the evaluated tools. Section \ref{sec:vulnerabilities} motivates our work and highlights the addressed challenges. Section \ref{sec:SolidiFI} discusses the general approach  of \sysname. \sysname's main algorithm and its implementation details are provided in Section \ref{sec:algorithm} and Section \ref{sec:imp} respectively. Section \ref{sec:eva} describes the experiments and results of using \sysname. Analysis and implications of the results are provided in Section \ref{sec:discussion}. Section \ref{sec:relWork} presents related work, and Section \ref{sec:conclu} concludes the paper.


==> SolidiFI-arXiv (2)/methodology.tex <==
\pdfoutput=1

\section{\sysname Approach and Workflow}
\label{sec:SolidiFI}

The main goal of \sysname is to perform systematic evaluation of \textit{static analysis} tools used to check smart contracts for known security bugs. Figure \ref{gprocess} shows the workflow of \sysname. 
The code snippets representing a specific security bug are injected in each smart contract's source code at {\em all} possible locations (step 1). The selection of the injection locations is a function of the bug to be injected. {\em \sysname injects bugs into the source code to imitate the introduction of bugs by developers. However, its use is not restricted to tools that perform analysis at the source code level. For example, tools that work on the EVM bytecode would compile the buggy contracts to produce the EVM code for analysis.} Then, the injected code is scanned using the static analysis tools (step 2). Finally, the results of each tool are checked, and false negatives and false positives are measured (step 3).

%Specifically, it focuses on  injecting faults (i.e., security bugs) in smart contracts, and then checking the injected code using the tools for cases that are not detected (i.e., false negatives).

\begin{figure}[h] 
\centering
\includegraphics[width=\columnwidth]{approach.png}
\caption{\sysname Workflow.}
\label{gprocess}
%\vspace{-5mm}
\end{figure}


\subsection{Bug Model}

In our work, a security bug is expressed as a code snippet, which leads to a vulnerability that the security tool being analyzed aims to detect. \sysname reads code snippets to be injected from a pre-defined bug pool prepared by us (the bug pool can be easily extended by users to add new bugs). For each tool, we only inject the bugs that the tool claims to detect. based on the tool's research paper. %, (2) online code repository, and (3) documentation. 
However, because the tools are continuously evolving,  the research paper may not have the up-to-date list of bugs detected by the tool, and hence we use the tool's online documentation to augment it. 

%\begin{enumerate}
 %   \item \textbf{Tool's research paper:} We consider the research paper of the tool as a primary source of information about the security bugs that the tool aims to detect. We formulate the code snippets and perform code transformation to inject the security bugs, based on the properties and examples of the bugs provided in the tool's paper. 
 %   \item \textbf{Tool's online repository:} The research paper may not have the complete or up-to-date list of the bugs addressed by the tool., either because of the continuous development of the tool or the space limitation of the paper. In addition, some tools do not have a corresponding research paper. Therefore, we search the online repository of the tool, if any, to find extra information about the bugs addressed by the tool.
%    \item \textbf{Tool's documentation:} This is the list of the bugs that are supposed to be detected as per the tool's main interface or online documentation.
%\end{enumerate}

\subsection{Bug Injection}
\label{buginstrument}
In this work, the security bugs are injected in the source code in three ways as follows.

\subsubsection{Full code snippet}
In this approach, we prepare several code snippets  for each bug under study. Each code snippet is a piece of code that introduces the security bug. %For some bugs, the bug can be formulated in more than one pattern or code snippet. 
To illustrate the process, we discuss the bugs and example code snippets. %how we formulate the related code snippets. 

\paragraph{\textbf{Timestamp dependency}}
The current timestamp of the block can be used by contracts to trigger some time-dependent events. Given the decentralized nature of Ethereum, 
%time can be synchronized by nodes to some degree. Although the miners cannot change the timestamp of their blocks to a value in the past (smaller than the previous one) or far ahead to the future, they 
miners can change the timestamp (to some extent). Malicious miners can use this capability and change the timestamp to favor themselves. This bug was exploited in the GoverMental Ponzi scheme attack \cite{EthereumAttacksHistory}. Therefore, developers should not rely on the precision of the block's timestamp. Figure~\ref{fig:timestamp-example} shows an example of a 
code snippet that represents  the bug (\textit{block.timestamp} returns the block's timestamp).

\begin{figure}[h]
\centering
\footnotesize
\begin{lstlisting}[language= Solidity, basicstyle=\ttfamily]
function bug_tmstmp() public returns(bool)
{   return block.timestamp >= 1546300;}
\end{lstlisting}
\caption{Timestamp dependency examples.}
\label{fig:timestamp-example}
%\vspace{-4mm}
\end{figure}

\paragraph{ \textbf{Unhandled exceptions}}
In Ethereum, contracts can call each other, and send \textit{ether} to each other (e.g., \textit{send} instruction, \textit{call} instruction, etc.). If an exception is thrown by the callee contact (e.g., limited gas for execution), the contract is terminated, its state is reverted, and  \textit{false} is returned to the caller contract. Therefore, unchecked returned values within the caller contract could be used to attack the contract, leading to undesired behavior. A serious version of this bug occurred in the ``King of the Ether" \cite{EthereumAttacksHistory}. Figure~\ref{fig:unhandled-exception-example} shows an example (the \textit{send()} instruction requires its return value to be checked for exceptions to make it secure).
% case in which a call is made without properly handling the exceptions - this is an example of the snippets we inject.
\begin{figure}[h]
\footnotesize
\centering
\begin{lstlisting}[basicstyle=\ttfamily]
function unhandledsend() public {
    callee.send(5 ether);}
\end{lstlisting}
\caption{Unhandled exceptions examples.}
\label{fig:unhandled-exception-example}
%\vspace{-4mm}
\end{figure}
 \paragraph {\bf Integer overflow/underflow} In Solidity, storing a value in an integer variable bigger or smaller than its limits lead to integer overflow or underflow. This can be used by attackers to fraudulently siphon off funds. For example, Figure \ref{fig:int-overflow-example} shows an example code snippet in which an attacker can reset the {\em lockTime} for a user by calling the function \textit{incrLockTime} and passing 256 as an argument - this would cause an overflow, and end up  setting the lockTime to 0. Batch Transfer Overflow is a real-world example \cite{PoWHC}.
 \begin{figure}[h]
 \footnotesize
\centering
\begin{lstlisting}[basicstyle=\ttfamily]
function incrLockTime(uint _sec) public{
        lockTime[msg.sender] += _sec;}
\end{lstlisting}
\caption{Integer overflow/underflow example.}
\label{fig:int-overflow-example}
%\vspace{-4mm}
\end{figure}

\paragraph {\bf Use of tx.origin} In a chain of calls, when contracts call functions of each other, the use of  {\em tx.origin} (that returns the first caller that originally sent the call) for authentication instead of {\em msg.sender} (that returns the immediate caller) can lead to phishing-like attacks \cite{solidity-security-blog}. Figure \ref{fig:tx.origin} shows an example snippet in which {\em tx.origin} is used to withdraw money. 
% from the contract.
\begin{figure}[h]
\footnotesize
\centering
\begin{lstlisting}[basicstyle=\ttfamily]
function bug_txorigin(address _recipient) public {
    require(tx.origin == owner);
    _recipient.transfer(this.balance);}
\end{lstlisting}
\caption{tx.origin authentication example.}
\label{fig:tx.origin}
%\vspace{-4mm}
\end{figure}

 \paragraph{\bf Re-entrancy} Contracts expose external calls in their interface. These external calls can be hijacked by attackers to call a function within the contract itself several times, thereby performing unexpected operations within the contract itself. For example, the external call in Line 3 of the snippet code shown in Figure \ref{fig:Re-entrancy} can be used by an attacker to call the {\em bug\_reEntrancy()} function repeatedly, potentially leading to withdrawal of ether more than the balance of the user. The DAO attack \cite{dao2017} is a well-known example exploiting this bug.
 % since the balance is updated at line 3 after sending the withdrawn amount.
 \begin{figure}[h]
 \footnotesize
\centering
\begin{lstlisting}[basicstyle=\ttfamily]
function bug_reEntrancy(uint256 _Amt) public {
  require(balances[msg.sender] >= _Amt);
  require(msg.sender.call.value(_Amt));
  balances[msg.sender] -= _Amt;}
\end{lstlisting}
\caption{Re-entrancy example.}
\label{fig:Re-entrancy}
%\vspace{-4mm}
\end{figure}
    %\item \textbf{Missing constructor:} In the old version of Solidity, a constructor is the function that hold the same name of the contract~\footnote{Recent versions of the Solidity compiler will check this at compile-time, and will not compile the contract if the consitructor is not present. However, the Mythril tool checks for this bug and hence we have included it. }. Changing the name of the constructor makes it available for public access.
\paragraph{\bf Unchecked send} Unauthorized Ether transfer, such as non zero sends, can be called by external users if they are visible to public, even if they do not have the correct credentials. This means unauthorized users can call such functions and transfer ether from the vulnerable contract \cite{solidity-security-blog}. An example code snippet is shown in Figure~\ref{fig:uncksend}.

\begin{figure}[h]
\footnotesize
\centering
\begin{lstlisting}[basicstyle=\ttfamily]
function bug_unchkSend() payable public{
      msg.sender.transfer(1 ether);}
\end{lstlisting}
\caption{Unchecked send example.}
\label{fig:uncksend}
%\vspace{-4mm}
\end{figure}

    
\paragraph {\bf Transaction Ordering Dependancy (TOD)} Changing the order of the transactions in a single block that has multiple calls to the contract, results in changing the final output \cite{atzei2017survey}. Malicious miners can benefit from this. An example code snippet vulnerable to this bug is shown in Figure~\ref{fig:tod}. In this example, the attackers can send a puzzle solving reward to themselves instead of the winner of the game by executing {\em bug\_tod2()} before {\em bug\_tod1()}.
\begin{figure}[h]
\footnotesize
\centering
\begin{lstlisting}[language= Solidity, basicstyle=\ttfamily]
address payable winner_tod;
function setWinner_tod() public {
    winner_tod = msg.sender;}
function getReward_tod() payable public{
    winner_tod.transfer(msg.value);}
\end{lstlisting}
\caption{TOD example.}
\label{fig:tod}
%\vspace{-4mm}
\end{figure}


%\paragraph {\bf Denial of Service(DoS) by an external contract} Contracts sometimes depend on an external call to transition to a new state. In this case, the failure of the external call can lead to DOS attacks \cite{solidity-security-blog}. An example code snippet is shown in Figure \ref{fig:dos}. The GoverMental Ponzi scheme attack exploited DoS vulnerabilities \cite{EthereumAttacksHistory}.

%\begin{figure}[h]
%\footnotesize
%\centering
%\begin{lstlisting}[basicstyle=\ttfamily]
%function dos(address Addr, address winner) public 
% { if (Addr.answer () < 42) 
% { winner= msg.sender; }}
%\end{lstlisting}
%\caption{DoS by external contract example.}
%\label{fig:dos}
%\end{figure}

\subsubsection{Code transformation}
This approach aims to transform a piece of code without changing its functionality, but make it vulnerable to a specific bug. We leverage known patterns of vulnerable code to inject this bug. We use this approach to inject two bug classes that are compatible with this approach, namely (1) integer overflow/underflow and (2) use of tx.origin. 
%However, \sysname allows end-users to define their patterns for injecting new bugs. 
%Although we are using it with two bug types, \sysname was deigned to be generic and allows the tool users to define their own patterns for other bug types. 

Table \ref{tab:codetranformpattern} shows examples of the code patterns that are replaced to introduce the bugs, and the vulnerable patterns for each bug type.

\begin{table}[h]
\begin{center}
\caption{Code transformation patterns.}
\begin{tabular}{|c|c|c|}  
\hline
 \textbf{Bug Type}&{\textbf{Original Code Patterns}}&{{\textbf{New Code Patterns}}} \\
\hline
tx.origin&msg.sender==owner& tx.origin==owner\\
%\hline
%Integer overflow&unit&int\\
\hline
Overflow&bytes32&bytes8\\
\hline
Overflow&uint256&uint8\\
\hline

\end{tabular}
\label{tab:codetranformpattern}
\end{center}
%\vspace{-4mm}
\end{table}

% For example,
%we could replace all instances of \textit{transfer} function with the less secure \textit{send} or \textit{call} functions, or look for calls to specific functions and reduce the parameter values. 
Figure \ref{fig:code_trans_example}  shows an example before and after bug injection using this approach. In this example, \textit{transfer} instruction is used to perform a transfer of the specified ether amount to the receiver's account after verifying the direct caller of \textit{sendto()} to be the owner. To inject the tx.origin bug, the authorization condition \textit{msg.sender == owner} should be replaced with the \textit{tx.origin == owner}, in which the owner is not the direct caller of \textit{sendto()}. However, the authorization check is passed successfully, which enables attackers to authorize themselves, and send ether from the contract, even if they are not the owner.

\begin{figure}[h]
\centering
\footnotesize
\begin{lstlisting}[basicstyle=\ttfamily]
/*(Before)*/
function sendto(address receiver, uint amount) public  {
    require (msg.sender == owner);
    receiver.transfer(amount);}
/*(After injection)*/
function sendto(address receiver, uint amount) public {
    require (tx.origin == owner);
    receiver.transfer(amount);}
  \end{lstlisting}
 \caption{Code transformation example.}
 \label{fig:code_trans_example}
 %\vspace{-6mm}
\end{figure}

\subsubsection{Weakening security mechanisms} 
In this approach, we weaken the security protection mechanisms in the smart contract code, which protect external calls. Note that our goal is to evaluate the static analysis tool, and not the smart contract itself. %For example, we remove the revert statements that are used  after failures of ether  transfer or calling another contract.
 We use this approach to inject Unhandled exception bugs. 
 Figure~\ref{fig:weakening-example} shows an example, in which the  \textit{Unhandled exceptions} bug is injected by %weakening the security checks of balance withdrawal by 
 removing the {\em revert()} statement that reverts the state of the contract if the transfer transaction failed - this causes the balance to incorrectly become 0 even if the transaction failed.

\begin{figure}[h]
\centering
\footnotesize
\begin{lstlisting}[basicstyle=\ttfamily]
/*(Before)*/
function withdrawBal () public{
  Balances[msg.sender] = 0;
  if(!msg.sender.send(Balances[msg.sender]))
    { revert(); }}
/*(After injection)*/
function withdrawBal () public{
  Balances[msg.sender] = 0;
  if(!msg.sender.send(Balances[msg.sender]))
    { //revert();
    }}
\end{lstlisting}
\caption{Weakening security example.}
\label{fig:weakening-example}
%\vspace{-4mm}
\end{figure}



==> SolidiFI-arXiv (2)/motivation-challenges.tex <==
\pdfoutput=1

\section{Motivation and Challenges}
\label{sec:vulnerabilities}

This section first presents motivating examples of undetected security bugs by static analysis tools, followed by an overview of the challenges in the evaluation of the tools.

\subsection{Motivating examples}

The contract example in Figure \ref{fig:example-contract} has at least 2  vulnerabilities, (1) two instances of timestamp dependency bug at lines 8 and 12, and (2) one instance of transaction ordering dependence (TOD) represented by the transactions at lines 13 and 16. 
The timestamp dependency bug is that the block's timestamp should not be used in the transaction, while the TOD bug is that the state of the smart contract should not be relied upon by the developer (Section~\ref{sec:eva}).

We have used four of the static analysis tools in Section~\ref{sec:background} (supposed to detect these bugs) to check this contract for bugs, Oyente, Securify, Mythril, and SmartCheck. According to the tools' research papers \cite{luu2016making, tsankov2018securify, mueller2018smashing, tikhomirov2018smartcheck}, Oyente, Mythril and SmartCheck should detect the timestamp dependency bug. 
However, we found that while Oyente and Mythrill were not able to detect both instances of timestamp dependency bug in lines 8 and 12,  Smartcheck detected only the instance in line 12. For the second instance, Smartcheck gave a hint that block.timestamp should be ``used only in equalities''. To further test SmartCheck's ability to detect the bug, we made a small modification to the syntax of the smart contract while keeping its semantics the same (Figure~\ref{fig:contract-modification}). SmartCheck subsequently failed to detect the bug altogether.
% and consisted of replacing line 11 with the 2 lines shown in the figure. The bug is not detected by SmartCheck, after the modification.

\begin{figure}
\footnotesize
\centering
\begin{lstlisting}[firstnumber=11]
  uint _vtime = block.timestamp;
  if (startTime + (5 * 1 days) == _vtime){
\end{lstlisting}
\caption{Modification made to the contract in Figure \ref{fig:example-contract}}
\label{fig:contract-modification}
\vspace{-3mm}
\end{figure}

Regarding the TOD bug, both Oyente and Securify are supposed to detect this class of bugs. 
However, we found that only Securify detected this bug successfully while Oyente was not able to detect it.
We extracted the code snippet representing TOD from this contract (lines 10 to 16), injected it in another larger contract free of bugs, and obtained similar results. 

These examples motivated us to prepare multiple code snippets for the different bugs (within the scope of the tools) and to manually inject them into the code of 5 smart contracts (the first 5 contracts in the set of contracts in Section~\ref{sec:eva}). We then used the tools to check the buggy contracts, and found several instances of undetected bugs even though the tools were supposed to detect them. However, it was tedious and error-prone to manually inject these bugs and inspect the results, and so we decided to automate this process. %, which is the main motivation for our work in this paper. 
%, and used the four tools to check the new buggy contracts. By inspecting the tools' results, we were able to find several undetected instances of bugs belonging to different bug types. The results of our manual injection inspired us to the fact that it would be useful to use bug injection to build a systematic approach for evaluating smart contract security analysis tools, which is the scope of our work in this paper.

\subsection{Automated bug injection challenges}
\label{injectionchallenges}

The simplest way to inject bugs into smart contracts is to inject them at random locations - this is how traditional fault injection (i.e., mutation testing) works. However, random injection is not a cost-effective approach as we have to follow specific guidelines for the injected bug to be exploitable. We identify two main challenges.

\subsubsection{Bug injection locations}
As the underlying techniques used by some tools (e.g., symbolic execution) depends on the control and data flow in the analyzed contracts, injecting an instance of each bug at a single location would not be sufficient. Therefore, bugs should be injected into all potential locations in the contract code. On the other hand, the process of identifying the potential locations depends on the code of the original contract, and also on the type and nature of each bug. Injecting bugs at the wrong locations would result in compilation errors. In addition, it might yield instances of dead code in the contract. For example, injecting a bug formulated as a stand-alone function inside the body of another function would result in a compilation error, as Solidity does not support nested functions. 
Moreover, a bug injected into an 'if' statement condition  that would make the condition always fail, would make the 'then' clause unreachable.
 
\subsubsection{Semantics dependency}
For the injected bug to be an active bug that can be exploited by an attacker, it has to be aligned with the semantics of the original contract. %For example, the syntax of an injected bug might be correct; however, it may not be executed due to its dependency on some other environment variables that are not applicable in the original contract being injected. 
For example, assume that we want to inject a Denial of Service (DoS) bug by calling an external contract. We can use an if-statement with a condition containing a call to another contract function. However, for this bug to be executed, we also need to define the appropriate external contract.

%\karthik{Results inspection seems more like an engineering challenge, not a research challenge}
%\subsubsection{Results inspection}
%In addition to automating the injection process, there is a need to automate the results inspection process to generate a list of the undetected faults automatically. However, automating the results inspection is challenging due to the inconsistency of the generated reports, as each tool uses its own custom format and provides different information. In addition, some tools provide incorrect information, such as the location of the detected bug, that cannot be matched with the analyzed contract. For instance, the locations associated with the detected bugs returned by Mythril do not match the actual locations in the source code.

\sysname addresses the first challenge by parsing the Solidity language into an Abstract Syntax Tree (AST) and injecting bugs into {\em all} syntactically valid locations. It addresses the second challenge by formulating exploitable code snippets for each bug type.
% which can be exploited by an attacker.

==> SolidiFI-arXiv (2)/related_work.tex <==
\pdfoutput=1

\section{Related Work}
\label{sec:relWork} 
%To the best of our knowledge, \sysname is the first work for evaluating smart contract static analysis tools using bug injection. 
%In this section, we survey related work in two areas.

\textbf{Bug-finding Tools Evaluation}
The approach of injecting bugs for evaluating the effectiveness of bug finders has been applied in other contexts than smart contracts.
%in other fields than smart contracts such as mobile applications and traditional programs.
Bonett et al. proposed $\mu$SE \cite{bonett2018discovering}, a mutation-based framework for the evaluation of Android static analysis tools that works as follows. First, a fixed set of  security operators are created describing the unwanted behavior that the tools being evaluated aim to detect (e.g., data leakage). 
Then, $\mu$SE inserts the security operators into mobile apps based on mutation schemes, that consider Android abstractions, tools reachability and security goals of the tools, thereby creating multiple mutants that represent unwanted behavior within the apps. 
The mutated apps are analyzed using the static tools to be evaluated. However, unlike our work, the undetected mutants are analyzed manually. Further, their framework focuses only on data leak detection tools, unlike our work, which is more general.

Pewny et al. \cite{pewny2016evilcoder} automatically find potential vulnerable  locations in C code, and modify the source code to make it vulnerable. Program analysis techniques are used to find sinks in the programs matching specific bug patterns, and find connections to user-controlled sources through data-flow. The program is modified accordingly to make it exploitable. In contrast to our approach, the vulnerable code locations to be injected are randomly chosen, and the implemented prototype targets the injection of spatial memory errors through the modification of security checks.% The injection through removing and modifying security mechanisms on the identified paths between sinks and user-controlled sources may not be sufficient for creating exploitable vulnerabilities. 

Dolan-Gavitt et al. \cite{dolan2016lava} proposed LAVA for generating and injecting bugs into the source code of programs using dynamic taint analysis. A guard is inserted for every injected bug for triggering the vulnerability if a specific value occurs in the input. Specifically, LAVA identifies an execution trace location where an unmodified and dead input data byte (DUA) is available. Then code is added at this location to make the DUA byte available, and use it execute the vulnerability.
% DUAs are identified by running the program for specific inputs under dynamic taint analysis. 
Unlike our work, the injection is based on dynamic taint analysis, and the injected bugs are accompanied by triggering inputs. In contrast, our goal is to transform invulnerable code to systematically introduce vulnerabilities in it.

In recent work, Akca et al. \cite{akca2019solanalyser} proposed a tool that the authors used to compare the effectiveness of their introduced smart contracts static analyzer with some other tools. by injecting a single bug into the contract code. Unlike our approach that injects exploitable bugs into all potential locations in the contract code, the tool uses Fault Seeder \cite{peng2019sif} to generate contract mutants by injecting only a single bug snippet (hard-coded in the source code) into a specific location in the smart contract. In addition, the authors conducted manual inspection of the tool reports to determine false negatives. Injecting a single bug does not provide a comprehensive coverage evaluation of static analysis tools. Also, it is not clear how to evaluate the efficacy of static analysis tools on detecting deep vulnerabilities and corner cases by injecting only a single bug. As presented before, each bug can be introduced in the code in several ways, in this case, injecting a single-bug will not test the efficacy of the static analysis tools to detect various variants of each bug.

Durieux et al. \cite{durieux2019empirical} compared a number of smart contract static analysis tools. Unlike our work, the evaluation is based on using 69 manually annotated smart contracts with 112 bugs in total. The vulnerable contracts are collected from online repositories that are not agnostic of the evaluated tools, hence, results might be biased (e.g., collecting 50\% of the contracts from SWC Registry referenced by Mythril and maintained by the team behind it). In contrast, our goal is to perform systematic and comprehensive coverage evaluation of static analysis tools by transforming invulnerable code to systematically introduce vulnerabilities into all valid locations. We evaluated 6 tools on detecting about 9369 distinct bugs. To provide a fair evaluation of the tools, we evaluate each tool only on the bugs that it is designed to detect. Our proposed approach can be easily used to evaluate smart contract static analysis tools for detecting other bug types. Further, it enables end-users to choose any dataset of smart contracts for evaluating the tools.


\textbf{Smart Contract Testing and Exploitation}:
%In the space of smart contracts testing, few works have been proposed recently with the aim of generating test cases for smart contracts. 
There have been many recent papers on testing smart contracts, and automatically generating security exploits on them.
Wu et al. \cite{wu2019mutation} produce test cases by mutating specific patterns in smart contracts.
Chan et al. \cite{chan2018fuse} develop a fuzz testing service (Fuse) to support the fuzz testing of smart contracts. This is a work in progress report, and only presents the architecture of the fuzz service being developed. Wang et al. \cite{wang2019towards} target the generation of test suites for smart contracts. This work guides automatic generation of test cases for Ethereum smart contracts.
Eth-mutants \cite{eth-mutants} is another mutation testing tool for smart contracts. However, it is limited to replacing $<$ to $\leq$, and $>$ to $\geq$ (and vice versa).
%Another attempt for developing a mutation tool for smart contract was proposed in 2016 \cite{mutationattempt} with no progress in this attempt. 
Unlike our focus on evaluating smart contracts' static analysis tools, these papers target the generation of test cases for the smart contracts.
%In the space of smart contracts analysis, several approaches have been proposed based on static analysis techniques for ensuring security of Ethereum smart contracts. Most of those approaches are based on symbolic execution \cite{king1976symbolic}. Similar to Oyente \cite{luu2016making} and  Mythril \cite{mueller2018smashing}, Manticore \cite{manticore} also employs symbolic execution to detects bugs by extracting execution paths that satisfy a specific property. EthIR \cite{albert2018ethir}, an extension of Oyente, performs high-level analysis of EVM bytecode and simplifies the analysis by generating an intermediate rule-based representation where local variables are introduced into each basic block. Maian \cite{nikolic2018finding} extends the same approach adopted in Oyente to identify three classes of trace vulnerabilities using a pattern-based approach. Unlike Oyente that models the behavior of a single call in a contract, Maian considers a sequence of invocations of the contract. 

%A number of static analyzers address the issue of path explosion and scalability  when using symbolic execution \cite{tsankov2018securify, grech2018madmax, grech2018madmax}. Securify \cite{tsankov2018securify} and Madmax \cite{grech2018madmax} avoid path explosion by approximating and merging relevant execution paths. ZEUS \cite{kalra2018zeus} translates the source code of a smart contract along with a policy specification into LLVM bitcode, an intermediate representation (IR), which is fed to a verification engine to check the safety of the smart contract. Some of the analyzers are based on converting the EVM bytecode to IR that is easier to analyze such as Vandal \cite{brent2018vandal} and Erays \cite{zhou2018erays}. Vandal converts EVM bytecode to logical relations that indicates the smart contract's semantics. Then those logic relations are analyzed to detect vulnerabilities described in the Souffle language. The reverse engineering tool, Erays, produces high-level pseudocode from EVM bytecode that is suitable for manual analysis. 
%\karthik{Rather than go into the details of these approaches, say why your approach is different?}

%In contrast to static analysis approaches, ECF \cite{grossman2017online} performs dynamic monitoring of smart contracts. ECF introduces a dynamic checker to identify reentrancy bugs. It dynamically checks effectively callback free (ECF) objects in a given execution trace, and statically checks if an object is ECF.

Other papers focus on automatic exploitation of smart contracts to generate exploits or malicious inputs to exploit found code vulnerabilities \cite{krupp2018teether, jiang2018contractfuzzer, Feng2019smartscopy}.  teEther \cite{krupp2018teether} generates exploits for vulnerable contracts using symbolic execution with the Z3 constraint solver \cite{z3} to solve path constraints for the critical paths in the control flow graph. Contractfuzzer \cite{jiang2018contractfuzzer} uses the Application Binary Interface (ABI) specifications of vulnerable smart contracts to generate exploits (fuzzing inputs) for two vulnerabilities. SMARTSCOPY \cite{Feng2019smartscopy} also synthesizes adversarial contracts for exploiting vulnerabilities in contracts based on ABI specifications of the contracts covering larger set of vulnerabilities than Contractfuzzer. Echidna \cite{echidna}  has been proposed for fuzzing smart contracts. It supports grammar-based fuzzing to generate transactions to test smart contracts. The goal of these techniques is testing the smart contracts themselves for security vulnerabilities rather than testing bug-finding tools.

==> implementation.tex <==
\pdfoutput=1

\section{\sysname Algorithm} 
\label{imp}
This section explains the  main algorithm of \textit{\sysname}. 
The process of evaluating static analysis tools by injecting bugs in a smart contract source code goes through four steps:
\begin{enumerate}
    \item Compile a version of the target contract and generate the Abstract Syntax Tree (AST).
    \item Use the generated AST to identify the potential locations for injecting bugs and generate an annotated AST marking all identified locations.
    \item Inject bugs into the marked locations to generate the buggy contract.
    \item Check the buggy contract using the evaluated tools and inspect the results for undetected bugs.
\end{enumerate}

The four steps are depicted in Figure \ref{fig:solidifi}, and Algorithm \ref{alg:solidifi} provides a high-level description of \sysname procedure for evaluating static analysis tools.

\begin{figure}[h] 
\centering
\includegraphics[width=0.75\columnwidth]{figures/solidifi.eps}
\caption{\sysname Components}
\label{fig:solidifi}
\end{figure}

\small
\begin{algorithm}[h]
\caption{\sysname High-level Algorithm}
\label{alg:solidifi}
\begin{algorithmic}[1]
\Procedure{main}{}
\State $AST \gets Parser(contract.sol)$
\For{Each bug type}
\State $FIP \gets Find All Potential Locations(AST)$
\For{Each location in FIP}
 \State{Decide injection approach}
 \If{approach  == inject snippet}
    \State{Inject matching bug snippet}
  \ElsIf{approach  == weaken security}
  \State{Weaken existing security mechanism}
  \ElsIf{approach  == transform code}
    \State{Do required code transformation}
  \EndIf
 \State{Record injection details in BugLog}
 \EndFor
 \EndFor
 \For{Each tool being evaluated}
  \State $Result \gets Check(buggyContract)$
  \State $Undetected Bugs \gets Inspect(result)$
 \EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}
\normalsize

\textbf{Abstract syntax tree generation:}
First, \sysname reads the source code of the target contract and compiles it to make sure it is a compiled version. Then abstract syntax tree (AST) of the  target contract is generated (line 1 in Algorithm \ref{alg:solidifi}).

\textbf{Bug locations identification:}
The generated AST is passed to \textit{Bug Locations Identifier}, that drives a bug injection profile (BIP) of all possible injection locations in the target contract for a given security bug (line 4 in Algorithm \ref{alg:solidifi}). FIP is derived using AST-based analysis for identifying potential injection locations in smart contract code. The process of identifying the possible locations for injecting a specific bug in the target contract depends on specific rules that specify the relation between the nature of the bug to be injected and the target contract structure. In general, bugs take two forms: an individual statement and a block of statements. A block of statements can be defined either as a stand-alone function or non-function block such as if statement. Therefore, we use a rule for each form of the bugs that defines the specifications of the locations in which the injection would be possible. For example, the specifications of the locations for injecting a bug formulated as a stand-alone function would be any location that is within the body of the contract and not inside the body of another function or conditional statement. \karthik{Can you show the actual rule - is it written as a grammar?}

\textbf{Bug injection and code transformation:}
\sysname uses a systematic approach toward injecting bugs into the potential locations in the target contract (lines 6-13 in Algorithm \ref{alg:solidifi}). The \textit{AST Transformer} model seeds a bug for each location specified in the FIP. It uses AST-based code transformation to modify the code. 
Three different approaches are used to inject bugs as discussed in Section \ref{buginstrument}.

In addition to injecting bugs in the target contract, \textit{Bug Injector} generates a \textit {BugLog} that specifies a unique identifier for each injected bug, and the corresponding location/s in the target contract where it has been injected (line 14 in Algorithm \ref{alg:solidifi}). The \textit{BugLog} is used for performing automated inspection of the scan results generated by the evaluated tools, to find a list of the injected bugs that were not detected.

\textbf{Buggy code check and results inspection:}
The resulting buggy contract is passed to the \textit{Tool Evaluator} that check the buggy code using the tools under evaluation (line 18 in Algorithm \ref{alg:solidifi}). It then scans the results generated by the tools looking for the bugs that were injected but undetected, with the help of \textit{BugLog} generated by the \textit{Bug Injector} (line 19 in Algorithm \ref{alg:solidifi}). A list of undetected bugs is the output of \sysname.

\section{Implementation}
\sysname uses Solidity compiler \textbf{solc} (mainly version 0.5.8) to compile the original source code file to make sure it is free from compilation errors before it is injected. In addition, \sysname uses \textbf{solc} to generate AST of the original code in json format. We have implemented the other components of \sysname in Python in about 435 lines of code. Those components are responsible for identifying the potential locations for injection, injecting bugs using suitable injection approach, and generating the buggy contract. In addition to implementing the component responsible for inspecting the results of the evaluated tools and then reporting the undetected bugs. 
